OBDA Constraints for Effective Query Answering (Extended Version)

In Ontology Based Data Access (OBDA) users pose SPARQL queries over an ontology that lies on top of relational datasources. These queries are translated on-the-fly into SQL queries by OBDA systems. Standard SPARQL-to-SQL translation techniques in OBDA often produce SQL queries containing redundant joins and unions, even after a number of semantic and structural optimizations. These redundancies are detrimental to the performance of query answering, especially in complex industrial OBDA scenarios with large enterprise databases. To address this issue, we introduce two novel notions of OBDA constraints and show how to exploit them for efficient query answering. We conduct an extensive set of experiments on large datasets using real world data and queries, showing that these techniques strongly improve the performance of query answering up to orders of magnitude.

==> 3-usecase.tex <==
%!TEX root = main.tex

\section{Challenges of OBDA in \statoil}
\label{sec:usecase}

In this section we briefly describe the real-world scenario we have
examined at \statoil,
and the challenges it presents for OBDA.\footnote{
We provide a more detailed description 
of the Statoil scenario without technical details in a submission to the in-use track.
Neither the techniques presented here nor the  results obtained with these techniques are included in that submission.
}
%
At \statoil,  users   access several databases  on a daily basis, but in this work
we focus on  the Exploration and Production Data Store (EPDS).
%
EPDS is  a large legacy SQL (Oracle 10g) database 
comprising over 1500 tables (some of them with up to 10 million tuples) and 1600 views. 
%
The complexity of the SQL schema of EPDS is such that it is
counter-productive and error-prone to manually write queries over the
relational database. 
Thus, end-users  use only a set of tools with
predefined SQL queries to access the database.
When users do not find the answers in their tools,
the information needs are either left unanswered or passed on to IT
experts. The latter   use a combination of
pre-defined queries and data manipulation tools in order
to get the answer. This process can take weeks.
 

This situation triggered the introduction of 
OBDA in \statoil in the context of the \optique project~\cite{computer-optique}.
In order to test the OBDA setting at \statoil, 
the users provided  60 queries  (in natural language) that
are relevant to their job, and that cannot be easily performed at the moment.
From the vocabulary used in the users' queries the \optique
partners in Oslo and Rome handcrafted an ontology,
and  a set of mappings connecting  the relevant parts of EPDS and the ontology. 
This preliminary ontology contains 90 classes, 37
object properties, and 31 data properties; 
and there are more than 140 mappings.
Using this vocabulary they also built the  60 SPARQL queries
modeling the original query catalog in natural language.

Out of these 60 queries, 17 were timing-out after 20 min. 
Two common patterns that we could observe on the queries timing-out
were that:\\
%\begin{enumerate}
%
%\item\label{prb:join}
\emph{(1)} Users were asking for objects (such as wellbores) and several properties 
of those objects (such as  completion dates, and location) 
that are all mapped to the same view. 
Since these views do not contain keys, the semantic optimizations described 
in Section~\ref{sec:background} were not applied, and the resulting SQL
queries contained up to 9 (redundant) self-joins. \\
%\vspace{1ex}
%
%\item\label{prb:union} 
\emph{(2)} Several classes and properties used in the queries were completely defined
by the mappings (for that given OBDA setting), 
thus the inference, which is reflected as SQL unions in the translated queries,
did not bring new information.





To illustrate the above concepts 
we provide a running example
coming from the  \statoil scenario (simplified for the sake of clarity): 



\begin{example}
	\label{ex:intro}
	We focus on  two user queries whose SQL translations contain redundancies caused by the patterns
	mentioned above.
	The fragment of the ontology relevant to  these queries is: 	
	the class \textowl{:Wellbore}\footnote{A wellbore is a hole drilled for the purpose of 
	exploration or extraction of natural resources.},  its subclass \textowl{:ProductionWellbore}, and the properties 
        \textowl{:completionDate},  \textowl{:hasInterval} and \textowl{:is\-}\textowl{InWell}. 
        The class \textowl{:Wellbore} is the domain of these three properties.
     	These classes and properties are defined by
	mappings of the form:\\
	\centerline{Class(subject) $\leftarrow$ \texttt{sql}$_{class}$~~~~~~~~~~
	Property(subject,object) $\leftarrow$ \texttt{sql}$_{prop}$}\\
	%
	The SQL queries used in these mappings contain joins between several tables
	and complex filter expressions.
	Next we introduce a simplified version of the mappings
	linking  three predicates used in the running example  with the database.  
	\begin{lstlisting}[basicstyle=\ttfamily\scriptsize,mathescape,frame=none,frame=tb]
	$\owlind{:Wellbore-\{wellbore\_s\}} \ \owl{rdf:type} \ \owl{:Wellbore}$
	$\leftarrow \SQL{\SELECT{} wellbore\_s \FROM{}  wellbore}$ $\SQL{\WHERE{} wellbore.r\_existence\_kd\_nm = 'actual' }$

	$\owlind{:Wellbore-\{wellbore\_s\}} \ \owl{:isInWell} \
	\owlind{:Well-\{well\_s\}}$
	$\leftarrow \SQL{\SELECT{} well\_s, wellbore\_s \FROM{}  wellbore}$ $\SQL{\WHERE{} wellbore.r\_existence\_kd\_nm = 'actual' }$

	$\owlind{:Wellbore-\{wellbore\_s\}} \ \owl{rdf:type} \ \owl{:ProductionWellbore}$
	$\leftarrow \SQL{\SELECT{} w.wellbore\_s}$ $\SQL{\FROM{} wellbore w, facility\_clsn }$ $\SQL{\WHERE{} } $ ... complex-expression
	\end{lstlisting}

	The  DB views used to define all the terms in the running example are \textowl{wellbore}, 
	\textowl{facility\_clsn}, and 	\textowl{wellbore\_interval}.
	 
	%\almargen{explain overlap between wellbore and name, etc, and exact mapping Wellbore}
		
	\emph{Query with Redundant Unions: } 
	Consider a simple SPARQL query that returns all the wellbores.
	This query will return not only the wellbores mapped to the class
%concept
 \textowl{:Wellbore},
	but also the ones that can be inferred from the subclasses of \textowl{:Wellbore}
	and from the properties where \textowl{:Wellbore} is the domain or range.
	Thus, standard techniques for OBDA would translate the query   into
	an SQL query that intuitively has the following structure:
%	\begin{equation*}\label{eq:manyUnionsIntro}
%		\begin{array}{l}
\vspace{-3.5ex}
\begin{center}$			
	sql_1 {=} sql_{\owl{{:}Wellbore}}  {\cup}
        sql_{\owl{{:}ProductionWellbore}} {\cup} sql_{\owl{:isInWell}}
 {\cup}        sql_{\owl{:hasInterval}}    
	  {\cup}  	sql_{\owl{:completionDate}} 
$
\end{center}
\vspace{-0.5ex}
%	\end{array}
%	\end{equation*}
	%
%	where $\dom(\text{P})$ is the domain of the property $P$. 
	Each of the mappings involved 	in this query accesses 
	different tables with different filters,  
	however only $sql_{\owl{:Wellbore}}$ is needed. 
	The SQL $sql_{\owl{:Wellbore}}$ projects information from a DB view: $\texttt{wellbore}$ that
	contains  \emph{all} the wellbores in EPDS.
	
	
	\emph{Query with Redundant Joins:} 
	Now consider a  query that returns all the wellbores, together with
        two attributes: completion date and the well where it is contained.
	The SPARQL-to-SQL translation technique generates
	  an SQL query with the following structure:\\[-2ex]	
\centerline{$
		sql_2 = sql_1 \Join sql_{\owl{:completionDate}} \Join sql_{\owl{:isInWell}}$}
		
	All the  answers from $sql_2$ could also be retrieved from a projection over \texttt{wellbore}.
	This is because 
	(i) $sql_1$ could be simplified  to  $sql_{\owl{:Wellbore}}$; 
	(ii) all the queried information about wellbores  (dates and wells)  are in \texttt{wellbore};
	and (iii)  there is a single date/well for each wellbore (there is an implicit functional dependency). 
%	is a functional dependency between wellbores and dates and wells.
	%nor  $sql_{\owl{:completionDate}}$ and $ sql_{\owl{:isInWell}}$ contain foreign keys.
	The problem we highlight here is that this SQL query contains two redundant joins, 
	that in general cannot be removed without knowing  the view definition and/or 
	the domain.
$\hfill\Box$
\end{example}




This kind of data dependent redundancy cannot be detected and removed by the current   
structural and semantic optimizations.
Observe that not every self-join is redundant, and therefore 
not every self-join 
can be blindly removed.
Moreover, not every redundant join is a self-join. 
Therefore, we propose  a new {notion}, \emph{virtual functional dependency} in OBDA (c.f. Section~\ref{s:fds-in-obda}),  to characterize 
when these redundant joins 
can be removed by the semantic optimization techniques.
Analogously, to safely remove the redundant  unions described above 
we propose the  {notion} of \emph{exact mappings} (c.f. Section~\ref{sec:exact-mappings-obda}).


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> 4.3-forcingCTEs.tex <==
%!TEX root = main.tex

\subsection{Exact mappings and \vfd together}
\label{sec:forcingCTE}

In some cases, even after removing redundant joins,
the optimizing SQL  occurs in several unions in the translated SQL query.
When the optimizing SQL is complex
it is detrimental to performance to evaluate it several times in each union.
Moreover, there are scenarios where, because of its complexity, 
detecting and handling  the  optimizing SQLs
can be expensive for the OBDA query optimizer.
%The previous two tuning techniques do not improve the performance in scenarios where
%the DB schema information is enough for the semantic optimizations to take place,
%and where there are no exact predicates high in the hierarchy as in the \statoil use case.
This happens often in the  NPD scenario.
The following simplified example from NPD illustrates this:

\begin{example}[NPD Example]\label{ex:CTE1}
  Consider the fragment  of query 6 from the NPD benchmark~\cite{LRXC*15}:

  \ignore{
  \centerline{\scriptsize
    SELECT ?w ?n ?y WHERE
  }
  \centerline{\scriptsize {?w  \owl{rdf:type}  \owl{npd:Wellbore};
      \owl{npd:hasName}  ?n;
      \owl{npd:completionYear}  ?y.
    } 
  }
  }
  
  \begin{lstlisting}[basicstyle=\ttfamily\scriptsize,mathescape,frame=none,frame=tb]
SELECT ?w ?n ?y WHERE  {
?w $\owl{rdf:type}$  $\owl{npd:Wellbore}$;  $\owl{npd:hasName}$  ?n;    $\owl{npd:completionYear}$  ?y.   } 
  \end{lstlisting}
In NPD, properties \textowl{npd:completionYear}   and  \textowl{npd:hasName} 
are defined  by  3 mappings each of them
projecting the same attributes \textowl{id},  \textowl{name}, and \textowl{year}
from 3 different tables, for simplicity let us call them $A,B,C$.
The class \textowl{npd:Wellbore} is defined by 1 mapping using a table $E$.
In this scenario there is a \vfd  $S\mapsto^b \textowl{npd:completionYear},$ $\textowl{npd:hasName}$.
This \vfd is \textowl{npd:completionYear}-optimizable,
and the optimizing SQL is the union of $A,B,C$.  Detecting query 
containment of this type of queries to apply semantic optimization  
might not be efficient during query execution (recall that this problem is NP-hard),
and moreover, if this union has to be computed several times by the DB engine
it is detrimental to performance.
%The propertyis defined by 4 mappings, 
%projecting the attributes \textowl{id} and \textowl{name}
%from $A,B,C$ and a fourth table $D$.
%, that contains all the wellbores in $A,B,C$.
%Thus, the  SQL resulting from translating the query above contains the union of 12
%SQL queries, many of them redundant because of the overlap in the mappings
%of the two properties above ($A,B,C$).
\end{example}

% By looking at the shape of the mappings, one would observe
%that \textowl{npd:completionYear} can be re-defined by a mapping assertion
%whose source query is a union of three tables, that the same source
%query can be re-used to define a mapping assertion for \textowl{npd:hasName}
%that subsumes three of its mapping assertions.



We reduce these redundancies by using  the SQL99's Common Table Expressions (CTEs). 
CTEs work as temporary views declared as part of an \sql query. 
% that last the duration of the transaction, 
%and they are 
Using CTEs we generate exact predicates to reduce the number of mappings, 
and therefore the number of SQL unions.
However, if we simply define different CTEs for each class and property, as in~\cite{BienvenuOSX-ijcai13},
we will fall back to the performance problem that we had with the views in the EPDS scenario due to redundant joins. 
If in Example~\ref{ex:CTE1}  we create a CTE, $T$, as the union of $A,B,C$, and we define  \textowl{npd:hasName} and
\textowl{npd:completionYear}  using only $T$ without specifying any \vfd,  
we would  get a redundant self-join over $T$ in  the translation of the SPARQL query above.
In Section \ref{sec:npd-expr} we  empirically show that if we use this approach the performance of 
query-answering is the same or even worse 
than not applying any optimization and keeping the redundancy.
We avoid these redundant joins over CTEs by creating CTEs for optimizable  virtual functional dependencies
and applying the tuning technique from Section~\ref{sec:npd-expr}.




\begin{definition}\label{def:cteDef}
Let $P_1\dots P_n$  be properties in $\T$ and $t_d$ be the template used for the domain of $P_1\dots P_n$.
Let $S_{t_d} = S^1_{t_d}$ and  $S_{t_d}\mapsto^b{P_1\dots P_n}$ be a  $P_1$-optimizable \vfd
%Let $C$ be optimizable w.r.t. the domain of $P_1$ and $D_i$
%optimizable w.r.t. the range of $P_i$.
The CTE for $S_{t_d}\mapsto^b{P_1\dots P_n}$ is defined as:\\
%
\centerline{$\text{WITH VFD$_{P_{1}\dots P_n}$ AS }  sql_{1}(\vec{z})$}\\
%
The exact CTE mappings for $P_i$ is of the form:\\
\centerline{$P_i(t^i_d(x),t^i_r(y)) \leftarrow VFD_{P_{1}\dots P_n}$}
\end{definition}

The definition for path \vfd is analogous, and extending these definitions to include optimizable concepts is
straightforward. 

\begin{example}[NPD Example \#2]\label{ex:CTE2}
Let $S$ be the set of wellbores.
In our example we have a virtual functional dependency of the form $S\mapsto^b{\textowl{npd:hasName}, \textowl{npd:completionYear}}$. 
%Moreover, \textowl{Wellbore} is optimizable w.r.t. the domain of these both properties. 
The CTE for $T$ is defined as  follows:
%
\begin{lstlisting}[basicstyle=\ttfamily\scriptsize,mathescape,frame=none,frame=tb]
WITH  VFD$_{npd:hasName, npd:completionYear}$  AS ( SELECT *  FROM $(A \cup B \cup C  )$ )
\end{lstlisting}
\end{example}


Exact mappings from Definition~\ref{def:cteDef} 
are meant to replace the mappings for the classes and properties related to the \vfd
The translation from SPARQL to SQL remains the same with a single extra step, adding the CTEs
used in the resulting SQL query.

\begin{example}[NPD Example \#3]\label{ex:CTE3}
Using this approach, the\\ SPARQL query in Example~\ref{ex:CTE1} would 
be translated (using the \vfd and exact mappings tuning) 
into a SQL query of the form:
%
\begin{lstlisting}[basicstyle=\ttfamily\scriptsize,mathescape,frame=none,frame=tb]
WITH  VFD$_{npd:hasName, npd:completionYear}$  AS ( SELECT *  FROM $A \cup B \cup C $ )
SELECT wellb, name, date FROM VFD$_{npd:hasName, completionYear}\Join E$ 
\end{lstlisting}
Recall that this query was previously translated into a query 
with 9 unions, and each of these unions had  up to 3 joins. 
\end{example}



\begin{corollary}
Let $Q$ be a SPARQL query,  $(\T,\M,D)$ be an OBDA setting, and $v$ a \vfd in $G^{(\T,\M,D)}$.
Let $\M'$ obtained from $\M$ by replacing the mappings for predicates involved in $v$
by their exact CTE mappings (c.f. Definition~\ref{def:cteDef}).
Then the answer of $Q$ over $(\T,\M,D)$ 
is the same as the answer of $Q$  over $(\T, \M', D)$ with the extended (with CTE)
 SPARQL to SQL translation. 
\end{corollary}
	
\myPar{Implementation}	
This technique has not been fully implemented in \ontop. We leave it for future work.	
We do presented preliminary results on the performance by manually creating and adding the CTEs
to the SQL queries generated by \ontop.
See Sections~\ref{sec:ctewis} and \ref{sec:npd-expr}.




















\ignore{
\begin{lstlisting}[basicstyle=\ttfamily\scriptsize,mathescape,frame=none,frame=tb]
$\owlind{Wellbore-\{id\}} \ \owl{npd:name} \ \owlind{\{name\}} $
$\leftarrow \SQL{\SELECT{} * \FROM{} \ Tab1 \ UNION Tab2 \ UNION \ Tab3}$      

$\owlind{Wellbore-\{id\}} \ \owl{npd:completionYear} \ \owlind{\{year\}} $
$\leftarrow \SQL{\SELECT{} * \FROM{} \ Tab1 \ UNION \ Tab2 \ UNION Tab3}$
\end{lstlisting}

By taking this into account, one might not push the join inside the
union and consider the union itself as a temporary table. Let this
union be Tab1 \UNION{}  TWell be
the query defining \owl{npd:Wellbore}, This would
produce the following unfolding

\begin{lstlisting}[basicstyle=\ttfamily\scriptsize,mathescape,frame=none,frame=tb]
$\SQL{\SELECT{} * \FROM{} \ TWell \JOIN{} TName \JOIN{} Temp}$
$UNION$
$\SQL{\SELECT{} * \FROM{} \ TWell \JOIN{} Temp \JOIN{} Temp}$
\end{lstlisting}

where \texttt{TWell} and \texttt{TName} are the remaining views defining wellbore and
name, respectively, and \texttt{Temp} is defined as the union of
\texttt{Tab1}, \texttt{Tab2}, and \texttt{Tab3}.
}

	
\ignore{

 
The idea that we will discuss here is to use CTEs to group the mapping  for the same class/property (and template) 
into a unique mapping assertion whose \sql part corresponds to the union of the SQLs of the original mappings. 

Back to our example, the mappings assertions for \texttt{npd:name} and \texttt{npd:completionYear} have the following shape:
\begin{center}
  \begin{minipage}{0.4\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\scriptsize,mathescape,frame=none,frame=tb]
$\owlind{Wellbore-\{id\}} \ \owl{npd:name} \ \owlind{\{name\}} $
$\leftarrow \SQL{\SELECT{} * \FROM{}  wellbore\_shallow\_all}$

$\owlind{Wellbore-\{id\}} \ \owl{npd:name} \ \owlind{\{name\}} $
$\leftarrow \SQL{\SELECT{} * \FROM{}  wellbore\_development\_all}$

$\owlind{Wellbore-\{id\}} \ \owl{npd:name} \ \owlind{\{name\}} $
$\leftarrow \SQL{\SELECT{} * \FROM{}  wellbore\_exploration\_all}$      

$\owlind{Wellbore-\{id\}} \ \owl{npd:completionYear} \ \owlind{\{year\}} $
$\leftarrow \SQL{\SELECT{} * \FROM{}  wellbore\_shallow\_all}$

$\owlind{Wellbore-\{id\}} \ \owl{npd:completionYear} \ \owlind{\{year\}} $
$\leftarrow \SQL{\SELECT{} * \FROM{}  wellbore\_development\_all}$

$\owlind{Wellbore-\{id\}} \ \owl{npd:completionYear} \ \owlind{\{year\}} $
$\leftarrow \SQL{\SELECT{} * \FROM{}  wellbore\_exploration\_all}$     
\end{lstlisting}
\end{minipage}
\end{center}


By using a CTE defining the union of wlbShallow, wlbDevelopment, and wlbExploration one can use one single mapping for each of these two properties.
\begin{center}
  \begin{minipage}{0.4\textwidth}
    \begin{lstlisting}[basicstyle=\ttfamily\scriptsize,mathescape,frame=none,frame=tb]
$\owlind{Wellbore-\{id\}} \ \owl{npd:name} \ \owlind{\{name\}} $
$\leftarrow \SQL{\SELECT{} * \FROM{}  cteTable}$

$\owlind{Wellbore-\{id\}} \ \owl{npd:completionYear} \ \owlind{\{year\}} $
$\leftarrow \SQL{\SELECT{} * \FROM{}  cteTable}$     
\end{lstlisting}
\end{minipage}
\end{center}



The unfolding (modulo optimizations) will then reduce to a single SPJ query, namely

\begin{lstlisting}[basicstyle=\ttfamily\scriptsize, mathescape, frame=none,frame=tb]
$\SQL{\SELECT{} id, name, year \FROM{} wlbOverview A, cteTable B, cteTable C}$
$\SQL{\WHERE{} A.id=B.id=C.id}$
\end{lstlisting}

Although the unfolded query is substantially shorter than in the
original example (12 unions versus a single conjunctive query),
experimental results show that such a query does not perform any
better than the original long unfolding. 

This can be explained by the
fact that temporary tables created by CTEs do not have any index, and
this makes the cost of performing joins prohibitive. This is one of
the main reasons why CTEs have not been considered as a possible
solution to the unfolding explosion problem so far. However, it is
clear that the self-join in the query is redundant because of the
functional dependency $id \rightarrow name, year$, and therefore it
can be removed. Removing the self-join dramatically change the picture,
since experiments with \postgres showed that the CTE query without self-joins
is much more scalable than the original unfolding. In particular, the execution time
drops to a half of the original execution time already when the data instance is still relatively small ( npd\_50 \davide{calculate hw many rows} ) 




}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> 5.2-wisconsin.tex <==
%!TEX root = main.tex

\subsection{Wisconsin Benchmark}
\label{sec:wisconsin}
We setup an environment based on the Wisconsin Benchmark~\cite{wisconsin}.
This benchmark was designed for the systematic evaluation 
of data\-base performance with respect to different query characteristics.
% such as, 
%selectivity factor,  joins operations on sargable and 
%non-sargable attributes, etc.
The benchmark comes with a schema that is designed so one can quickly understand 
the structure of each table and the distribution of each attribute value.
This allows easy construction of  queries that isolate the features that need to be tested. 
The benchmark also comes with a data generator to populate the schema. 
Unlike NPD or EPDS, the benchmark database contains synthetic data that allows easily
specifying a wide range of retrieval queries.  
For instance, in NPD or EPDS  it is very difficult to specify a selection query 
with a 20\% or 30\% selectivity factor.
This  task becomes even harder when we include joins into the picture.

The benchmark defines a single table schema (which can be used to
instantiate multiple tables). The table, which we now call  ``Wisconsin table'', contains
16 attributes, and a primary key (\texttt{unique2})
with  integers from 0 to 100 million randomly ordered. 


\ignore{
 as shown in Figure~\ref{fig:wins}. 

\begin{figure}[htb]
\scriptsize
\center
\begin{alltt}
CREATE TABLE t
( 
    unique1 integer NOT NULL,
    unique2 integer NOT NULL PRIMARY KEY,
    two integer NOT NULL,
    four integer NOT NULL,
    ten integer NOT NULL,
    twenty integer NOT NULL,
    onePercent integer NOT NULL,
    tenPercent integer NOT NULL,
    twentyPercent integer NOT NULL,
    fiftyPercent integer NOT NULL,
    unique3 integer NOT NULL,
    evenOnePercent integer NOT NULL,
    oddOnePercent integer NOT NULL,
    stringu1 char(52) NOT NULL,
    stringu2 char(52) NOT NULL,
    string4 char(52) NOT NULL
)	
\end{alltt}
\caption{Wisconsin Benchmark schema description}
\label{fig:wins}
\end{figure}

%The data for each attribute is generated with a distribution 
%that allows to easily compute the
%degree of selectivity of SQL operations (in JOINs with conditions, WHERE
%clauses, cross products, unions). 

In particular, given a target number of 
rows N, the data for each attribute is generated as follows:
\begin{compactitem}
	\item \texttt{unique1}. Integers from 0 to N (sequential).
	\item \texttt{unique2}. Integers from 0 to N (randomly ordered)
	\item \texttt{stringu1}. A 6 character alphabetic string generated from unique1.
	\item \texttt{stringu2}. A 6 character alphabetic string generated from unique2.
\end{compactitem}
}
%
We refer the reader to~\cite{wisconsin} for details on the algorithm
that populates the schema.% \texttt{stringu1} and \texttt{stringu2}.



\myPar{Dataset}
We used Postgres 9.1, and  DB2 9.7  as \ontop backends. 
The query optimizers were left with the default configurations.
All the table statistics  were updated. 

%vacuumed and analyzed to avoid table bloating. 
%
For each DB engine we created a database, each with 10 tables:  
5 Wisconsin tables
% as described in Figure~\ref{fig:wins}
 ($\text{Tab}_i, i=1,\ldots,5$),  and 5 tables materializing the join of
the former tables. For instance, \texttt{\small view123} materializes the join 
of the tables \texttt{\small Tab1}, \texttt{\small Tab2}, and
\texttt{\small Tab3}.
Each table contains 100 million rows, and each of the databases
occupied ca. 400GB of disk space.
%one containing tables with  100.000 rows (ontowis\_100k) and one with  100M ($10^8$) rows (ontowis\_100m). 
%The 100M databases each occupied circa 420Gb of disk space.



%Due to the space limitation, we only show here the results for Postgres and DB2.
%The remaining results can be found in our technical report~\cite{techreport}.

\myPar{Hardware}
We ran the experiments in an HP Proliant server with 24 Intel Xeon CPUs
(144 cores @3.47GHz), 106GB of RAM and five 1TB 15K RPM HD. 
%Note that all queries were ran sequentially, and hence only
%one core was used at a time. 
\ontop was run  with 6GB Java heap space.
%
The OS is Ubuntu 12.04 64-bit edition. 
%in a Intel Core i5 (2.5 GHz-8GB RAM)

\medskip
In these experiments, we ran each query 3 times, and we averaged the execution times.
There was a warm-up phase, where we ran 4 random queries not belonging to the tests.


\ignore{
\paragraph{Queries:} 
All the query execution times presented here refer to the average of 3 executions.
\almargen{what do we say about warm up?}
}

\input{5.2.1-expr-MissingKeys}

\input{5.2.2-expr-exactMap}

\input{5.2.3-expr-wiscCTEs}



%\subsubsection{Summary}





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> 5.2.1-expr-MissingKeys.tex <==
%!TEX root = main.tex

\subsubsection{Evaluating the Impact of \vfd-based Tuning}

The experiments in this section measure the impact 
of optimization based on \vfds.
%providing  virtual functional dependencies.
Tuning based on branching \vfds and path \vfds produces the same
effect in the resulting SQL query, therefore, for concreteness we
focus on branching \vfd.  The performance gain for path \vfd is the
same.

Recall that we started studying this scenario because EPDS contains
thousands of views that lack primary/foreign keys, and some of them
cannot be avoided in the mappings.  This prevents OBDA semantic
optimizations to take place.

The following experiments evaluate the trade-off of using views or their definitions depending on:
\begin{inparaenum}[\it (i)]
	\item type of mappings (using views or view definitions);
	\item the complexity of the user query (\#~of SPARQL joins);
	\item the complexity of the mapping definition (\#~of SQL joins);
	\item the selectivity of the query;
	\item the \vfd tuning ON/OFF;
	\item the DB engine (DB2/PostgreSQL);
%	\item the dataset size.
\end{inparaenum}


In the following we describe the queries, mappings and the OBDA
settings used in the different experiments.

\myPar{Queries}
In this experiment we tested a set of 36 queries each varying on:
\begin{inparaenum}[\it (i)]
\item the number of SPARQL joins (1-3), 
\item SQL joins in the mappings (1-4),  and 
\item selectivity of the query (3 different values). 
\end{inparaenum}
%Since here we show only the 100M dataset.
%, we will only focus on 72 queries.
The SPARQL queries have the following template:\\
\begin{center}
\begin{minipage}{0.75\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\scriptsize,mathescape,frame=none,frame=tb]
SELECT ?x ?y  WHERE {
  ?x a ${:Class-n-SQLs}$ . ?x ${:Property_1-n-SQLs}$ ?y$_1$ . 
                     $\vdots$
  ?x ${:Property_m-n-SQLs}$ ?y$_m$. Filter( ?y$_m$ < k% ) }
\end{lstlisting}
\end{minipage}
\end{center}

where  \texttt{Class-n-SQLs} and \texttt{Property$_i$-n-SQLs} are classes and properties defined by mappings which source is either an SQL join of $n=1\dots4$ tables, or a materialized view of the join of $n$ tables. Subindex $m$ represents the number of SPARQL joins, 1 to 3.
Regarding the selectivity of $k\%$,	
we did the experiments with the following values:
\begin{inparaenum}[\it (i)]
\item $0.0001\%$  (100 results);
%\item $0.0005\%$ (500 results );
%\item $0.001\%$ (1.000 results);
%\item $0.005\%$  (5.000 results);
\item $0.01\%$ (10.000 results);
\item $0.1\%$ (100.000 results).
 \end{inparaenum}
These  queries  do not belong to the Wisconsin benchmark. 


\myPar{OBDA Specifications} 
We have two OBDA specifications, one where classes and
properties are populated using an SQL that use original tables with
primary keys (1-4 joins) ($K_1$); and a second one where predicates
are populated using materialized views (materializing 1-4 joins).
This second setting we tested with $\vfd$ optimization ($K_2$) and without
optimization ($K_3$).  In the first OBDA setting, all the property subjects
are mapped into the tables primary keys.  There are no axioms in the
ontology. All the individuals have the same template $t$.
% is always empty in this experiment.

\ignore{
\myPar{\vfd Specifications}
Each  set of 36 queries was tested against 3 different scenarios. 
%Each setting varies the type of mappings, and if the optimization is on/off.
\begin{compactitem}
	\item : Using the mapping based on the original tables.  
	\item : Using the mapping based on materialized views  with  
	\item Using the mapping based on materialized views without optimization.
	%\item  original tables: 1-4 joins  on string keys
	%\item  materialized views (materializing 1-4 joins  on String keys) 
%	\item Properties are mapped to SQL that used a materialized views (materializing 1-4 joins  on String keys) with  key
\end{compactitem}
}
 Let $S_t$ be the set of all individuals.
In $K_2$ there are  12 branching \vfds  of the 
form $S_t \mapsto^b{\textowl{:Property$_m$-n-SQLs}}$ for every $n=1\dots4$, $m=1\dots 3$. 
The optimizable \vfds contain intuitively the properties populated from the same view, that is,\\
\centerline{$S_t \mapsto^b{\textowl{:Property$_1$-n-SQLs},\textowl{:Property$_2$-n-SQLs},\textowl{:Property$_3$-n-SQLs}}$} \\
for $n=1\dots 4$.

%72 q * 3 run * 3 db * 3 set
%In total we run XXX queries.
 
 

\ignore{

\begin{example}
	
\begin{center}
\begin{minipage}{0.4\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\footnotesize,mathescape,frame=none,frame=tb]
 
SELECT ?x ?y  WHERE {
?x a  :2Tab1 . 
?x :Tab3unique2Tab3 ?y . 
Filter( ?y < 100 )
}
\end{lstlisting}
\end{minipage}
\end{center}
	
\end{example}
}

\myPar{Discussion and Results}
The  results of the experiments are shown in~ Figure~\ref{fig:FDResults}.
Each $q_{i/j}$ represents the query with $i$ SPARQL joins over properties
mapped to $j$ SQL joins. 

%The solid lines represent the SPARQL queries in $K_1$,
%the dotted lines  represent the SPARQL queries in $K_2$, and
%the dashed lines  represent the SPARQL queries in $K_3$.

There is almost no difference between the results with
different selectivity, 
so for clarity we averaged the run times over different selectivities.
%Thus, each point in the graph represent the average of the 
%3 run times of 3 different queries.
%we only show the average of each query with three different selectivities. 
Since the experiment was run three times, each point in the figure
represents the average of 9 query executions. 

The experiment results  in Figure~\ref{fig:FDResults} show that 
all the SPARQL queries perform better in $K_2$ than in $K_3$ in both DB engines.
%, 
%and even across data sizes~\cite{techreport}.
Moreover, in all cases queries in $K_2$  perform at least twice as fast as  the ones in $K_3$,
even getting close to the performance of $K_1$.

In \ontop-Postgres, the execution of the hardest SPARQL queries in
$K_1$  is 1 order of magnitude faster than in $K_2$. The execution of these queries in
$K_2$ is 4 times  faster than in $K_3$.
In \ontop-DB2, the performance gap between the SPARQL queries in 
$K_3$ and $K_2$ is smaller.
The SPARQL queries in
$K_1$  are slightly faster than the queries in $K_2$. The execution in
$K_2$ is 2 times  faster than in $K_3$.

In \ontop-Postgres and \ontop-DB2, the translations of the SPARQL
queries resulting from the $K_3$ scenario contain self-joins of the
non-indexed views that force
%the query planner of
 the DB engines to create hash tables 
for all intermediate join results which increases the start-up cost of the joins, and the overall execution time. 
One can observe that in both, \ontop-Postgres and \ontop-DB2, the number of SPARQL 
joins strongly affect the performance of the query in $K_3$.  
In both cases, the SPARQL queries
in $K_2$, because of our optimization technique,  get translated into a join-free SQL query
that requires  a single sequential 
scan of the unindexed view. However, the cost  of scanning the whole view to perform a 
non-indexed filter is still higher than the cost of
joins (nested joins in both) of the indexed tables in $K_1$.






 
 
 \begin{figure*}[t]
 \centering
%EXPERIMENTS
 \pgfplotsset{every tick label/.append style={font=\tiny}}
% \input{ExperimentPostgres}
% \input{ExperimentPostgresOneSelectivity}
 \input{graphs/ExperimentPostgresAvgSel}
% \input{ExperimentDB2}
%\input{ExperimentDB2OneSelectivity}
\input{graphs/ExperimentDB2AvgSel}
 
 
 
%LEGEND
\begin{minipage}{.90\textwidth}
	\centering
		\footnotesize{
			\ref{fig:wis-mk-joins} $K_1$ (Querying the tables directly)~~~ 
			\ref{fig:wis-mk-views_tuned} $K_2$ (Views with optimization enabled)~~~\\
			\ref{fig:wis-mk-views_no_keys} $K_3$ (Views no optimization)~~~
			%\ref{cincuenta} $\sigma_{50.000}$~~~
			%\ref{cien} $\sigma_{100.000}$ ~~~
			%\ref{quinientos} $\sigma_{500.000}$ ~~~
			}
\end{minipage}
\caption{Experiments showing the impact of the optimization technique based on \vfd}
\label{fig:FDResults}	
\end{figure*}



\ignore{


 \input{ExperimentMysql}
 }







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\ignore{
\paragraph{Observations in Experiments with Views}

\mysql implements only the \emph{nested loop} algorithm for realizing the join operation. A different approach is the \emph{Hash Join} algorithm, implemented both in \dbtwo and \postgres which, by exploiting a combination of analysis of the physical data and usage of the main memory, often significantly outperforms the \emph{nested loop} procedure. In particular, the \emph{Hash Join} allows for a fast join on columns which are not explicitly defined as keys, but that are keys in practice; this because an index for those columns is constructed on-the-fly and in the main memory, and therefore the only overhead is the phase of the index construction (one single table scan). Below we show the execution plan of \postgres:
}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:



==> 5.2.2-expr-exactMap.tex <==
%!TEX root = main.tex

\subsubsection{Evaluating the Impact of Exact Mappings}\label{sec:expr-exactMap}

% This tuning technique was driven by a scenario that arises in the Statoil use case.

% The redundancy happens when you have a 1

% Note that some redundancies can be eliminated by semantic query
% optimization (in particular exploiting Foreign key
% constraints). However, it is not always possible. 

In this test we evaluate the exact mapping tuning technique described in Section~\ref{sec:exact-mappings-obda}.
%This experiment is inspired by the use case in EPDS where exact mapping tuning technique helps.
This experiment is inspired by the use case in EPDS where tuning based on exact mapping can help (c.f. Section~\ref{sec:usecase}).
%
The following experiments evaluate the impact of the tuning depending on:
%The effects of the experiment depend on:
%
\begin{inparaenum}[(i)]
\item the complexity of the query (\# of SPARQL joins);
\item the selectivity of the query;
\item the number of specified  exact classes;
\item the DB engine (DB2/PostgreSQL). 
%\item The dataset size.
\end{inparaenum}


In the following we describe the tables, ontology, mappings, queries and
 exact predicate specifications used in the experiment. 
% These queries do not belong
% to the Wisconsin benchmark, and were crafted to evaluate the impact of
% the tuning techniques.


\myPar{OBDA Setting}
The ontology contains four classes
$A_1, A_2, A_3, A_4$, one object property $R$ and one data property
$S$.  The classes form a hierarchy\\
$A_1 ~\rdfssubclassof~ A_2$, $~ A_2 ~\rdfssubclassof~ A_3$, $A_3 ~\rdfssubclassof~ A_4$.
%\myPar{Mappings} 
The mappings for classes $A_i$ ($i=1,\ldots,4$) are
defined over the primary key of Tab$_i$ with different
filters, in such a way that each $A_i$ is exact. The mappings for $R$ and
$S$ are defined over the primary key column and another unique column (\texttt{unique1})
of Tab$_5$.


\myPar{Queries}
 In this experiment we tested 6
%\guohui{update needed}
queries ($q_1,\ldots,q_6$) 
%with increasing complexity. 
%They are 
varying on: (i) the number of classes and properties in the SPARQL (1-3) and (ii) the
classes used in the query.
% , and (iii) selectivity of the queries (3
% different filters). 
For instance, $q_3$ is 
\begin{center}
\begin{minipage}{0.45\textwidth}
\begin{lstlisting}[basicstyle=\ttfamily\scriptsize,mathescape,frame=none,frame=tb]
SELECT * WHERE {?x a :A3. ?x :R y. ?y a :A4. 
  OPTIONAL { ?x :S ?u . } OPTIONAL { ?y :S ?v . }. }
\end{lstlisting}
\end{minipage}
\end{center}
% Each query $q_{i/j}$ ($1\leq i\leq 3, 1\leq j\leq 4$) has $i$ classes and 
%are combined with the same three filters as in Section~\ref{}.


\myPar{Exact Concept Specifications}
We consider the following four exact concept specifications:
%
$E_0 = \emptyset$, 
$E_1 = \{A_1,A_2\}$, 
	$E_2 = \{A_1,A_2, A_3\}$,
$E_3 = \{A_1,A_2, A_3, A_4\}$.
%
Observe that $E_0$ corresponds to the case where no exact mapping tuning is applied.


\myPar{Discussion and Results} 
The  results of the experiments are shown
% is illustrated 
in Figure~\ref{fig:exact-map-left}. %The solid lines, dotted lines, dashed lines, and XXXX\almargen{fix} lines represent
%the SPARQL queries under $E_0,E_1,E_2$, and $E_3$ respectively.
The results show that the exact mapping tuning improves the performance of
all SPARQL queries in both database engines. In particular, under the full tuning
setting $E_3$, none of the queries time out (20 mins), and the hardest queries  perform orders of magnitude faster than in $E_0$ and even $E_1$.
%\guohui{q6 is timeout in ontop-DB2.}
%all the queries can be answered efficiently. 

The performance gain is the result of the elimination of redundant unions.  
For instance, under $E_0$, SPARQL query $q_3$ is translated into a SQL
query with 12 unions, but 11 of them are redundant; applying $E_3$ removes
all the redundant unions.

\ignore{
One can observe in both, \ontop-Postgres and \ontop-DB2, the selectivity in the SPARQL queries does play a role in the execution time (unlike in the \vfd case), 
and  the number of SPARQL Optionals ???????? \almargen{Complete!!!!!}
}

%\guohui{now only one selectivity is tested.}
% strongly affect the performance of the query.  

 \begin{figure*}[t]
   \centering
%EXPERIMENTS
 \pgfplotsset{every tick label/.append style={font=\tiny}}
 \input{graphs/exact-map-pgsql-left}
 \input{graphs/exact-map-db2-left}
%LEGEND
\begin{minipage}{.90\textwidth}
	\centering
		\footnotesize{
			\ref{e0} $E_0$ (No exact mappings)~~~ 
			\ref{e1} $E_1$ (1 exact mapping)~~~
			\ref{e2} $E_2$ (2 exact mappings)~~~
			\ref{e3} $E_2$ (3 exact mappings)~~~
			}
\end{minipage}
\caption{Experiments showing the impact of the tuning technique based on Exact Mappings}
\label{fig:exact-map-left}	
\end{figure*}

 
% \begin{itemize}
% \item Effect of SPARQL joins. The query answering time is heavily
%   influenced by complexity of the query. In particular, the queries
%   involving classes with deep hierarchy are difficult to answer.
% \item the selectivity of the query also clearly affect the performance.
% \item The effect of optimization is very clear, especially for the
%   hard queries with deep hierarchies.
% \item DB2 is in general slower than Postgres in this test. (\guohui{needs to understand why})
% \end{itemize}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> 5.2.3-expr-wiscCTEs.tex <==
%!TEX root = main.tex

\subsubsection{Evaluating the Impact of CTE Tuning}\label{sec:ctewis}
The experiments in this section measure the impact 
of using CTEs combining \vfds and exact mappings  as described in Section~\ref{sec:forcingCTE}.
For these tests we adapted the setting  in
Section~\ref{sec:expr-exactMap}. 
%In particular, the mappings for the
%classes were modified so that exact mappings optimization would no
%longer be possible, 
We introduced four new mappings for  $R$ and $S$ (two each)
% that, by
%means of three different mappings, pick values from three different
%partitions of the same table. 
and we guaranteed the presence of
a virtual branching functional dependency for $R$ and $S$. 
The CTE is  defined as specified in Section~\ref{sec:forcingCTE}.
% partitions.

We evaluate two SPARQL queries. Query $q_{A_1}$ uses the leaf class $A_1$ and 2 SPARQL joins,
and the query  $q_{A_4}$ using the
class $A_4$ with 3 sub-classes and 2 SPARQL joins.
Without CTE tuning, these queries are translated into SQL queries with 9 and
36 unions respectively. 
By using CTEs,  these queries are translated into SQL queries with 1 and 3 unions respectively.
Figure~\ref{fig:cte-tuning-npd-wisc} shows the results of the
experiment. The experiments were run for both DB2 and Postgres
($q_{A1}^d$, $q_{A1}^p$ refer to the execution time of query $q_{A1}$
on  DB2 and Postgres, respectively).
We ran the experiments with and without \vfd.
When we do not specify \vfd, the translated queries contain self-joins over the CTEs.
The results show that the execution time of the SQL translation
with CTEs  (CTE-\vfd and CTE)  are one order of
magnitude faster than the execution time of the standard SQL
translation. 

% Interestingly, even without removing redundant
%self-joins (CTE-Self) on the CTEs the execution time of the tuned
%queries is significantly faster than the execution time of standard translation.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> 5.3-npdExperiments.tex <==
%!TEX root = main.tex

\subsection{NPD Benchmark}\label{sec:npd-expr}

We have run experiments over the three hardest queries of the NPD
benchmark ($q_6$, $q_{11}$, and $q_{12}$) and specified for each of
these queries CTEs like the one considered in
Section~\ref{sec:forcingCTE}. 
Recall that tuning based on \vfds and exact mappings alone do not improve the performance 
of query answering in this scenario. 
The results are shown in
Figure~\ref{fig:cte-tuning-npd-wisc}. Experiments are carried
out on the NPD dataset whose size has been increased by ten times
using the data generator that comes with benchmark. The
experiments were run for both DB2 and Postgres ($q_6^p$, $q_6^d$ refer
to the execution time of query $q_6$ under Postgres and DB2, respectively)
on the machine described in Section~\ref{sec:wisconsin}. 

\begin{figure}[t]
  \centering
  \input{graphs/cte/npd_wisc_bars.tex}
  \caption{CTE Tuning on Wisconsin (left) and  NPD\_10 (right) LogScale }
  \label{fig:cte-tuning-npd-wisc}
\end{figure}

The experiment shows that the execution time of the SQL translation with
CTEs and \vfd (CTE-\vfd) is significantly
 lower (c.a. a half) than the execution time of the standard SQL
translation (No CTE). 
Moreover, the execution time of the SQL translation without \vfd 
 (CTE)  can be significantly higher (one order of magnitude for Postgres) than the
other translations. This is because the SQL translation contains self-joins over the CTEs. 

%, regardless the underlying database engine.  


==> detecting.tex <==
\section{Detecting Tuning Cases (0.5p)}\label{sec:detecting}

\subsection{Detecting Functional Dependencies}\label{sec:detectingvfd}

Lemmas~\ref{lm:brn} and~\ref{lm:pth} require that the properties (classes) in the same $\mathcal{T}$-mapping hierarchy share the same template. This situation, however, is quite unlikely to happen in practice, and in particular it does not happen in NPD nor in SLEGGE. 

In~\cite{techreport} we show how the restriction can be relaxed. The idea is that lemmas can be repaired if each predicate $P$ defined by $n$ mappings using different templates can be replaced by $n$ fresh predicates where each fresh predicate uses one single mapping for $P$. So, the conclusions can be lifted in the general setting and therefore it is possible to devise a procedure to automatically search for these dependencies.

Detecting dependencies in the general case might be inefficient, since there are many inclusions checks that need to be performed and each of those can be expensive. 
A simpler approach is to just consider those predicates that are defined by the same view or table through the mappings. 
In such a situation, what remains to check is the presence of the virtual branching or path functional dependency; 
because of Lemmas~\ref{lm:brn} and~\ref{lm:pth}, this check reduces to verifying the presence of a functional dependency over the view. This can be performed by a single scan of the view.

\subsection{Detecting Complete Classes/Properties}
\label{sec:mining-exact}
Definition~\ref{dfn:exactmapping} implies that an exact mapping with respect to a particular data instance can be found by asking for all the individuals of the predicates defined by the vocabulary of the ontology over the virtual instances exposed by both input mappings and $\T$-mappings, and then comparing the results. 
By observing that OWL 2 QL is monotone (that is, adding $\T$-mappings cannot reduce the number of individuals for any predicate in the vocabulary) 
the comparison amounts to a simple cardinality check over the sizes of the results sets.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> graphs/ExperimentMysql.tex <==
%!TEX root = main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% LAST TESTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{
\begin{figure*}[tbp]
  \caption{ Davide: Final Recap Int }
  \input{graphs/graph-mysql-int.tex}
\end{figure*}

\begin{figure*}[tbp]
  \caption{ Davide: Final Recap Str }
  \input{graphs/graph-mysql-str.tex}
\end{figure*}
}

==> graphs/ExperimentPostgres-old.tex <==
%!TEX root = main.tex

\almargen{
E quindi qui siamo\cite{LRXC*15}
}
























\almargen{we need to re-do these experiments-commented}

\ignore{
\begin{figure*}[bth]
	
	\begin{tabular}{c}
	
	\begin{tabular}{cc}
		\begin{minipage}{.30\textwidth}
		\begin{tikzpicture}
		\pgfplotsset{every axis/.append style={
			font=\footnotesize,
			semithick,
			tick style={thick}}}
			% FishMark - Results
		    \begin{axis}[
				title= Postgres Pumped Int,
	    			height=7cm,
				width=14cm,
				xtick={0,1,2,3,4,5,6,7,8,9,10,11,12},
				xticklabels={0,1,2,3,4,5,6,7,8,9,10,11,12},
		        	grid=major,
				ymode=log,
				% legend to name=benchmarkset,
				legend columns=-1
		    ]
%%%%%%%%%%%%%%%%%%%%%%%    
   	     %JOINS !!
%%%%%%%%%%%%%%%%%%%%%%%
\addplot[black,mark=square,  mark options={solid}] coordinates {
(1,36463)(2,56721)(3,63524)(4,39960)(5,50929)(6,62401)(7,41697)(8,59913)(9,61102)(10,46885)(11,49938)(12,52916)
};
 \label{mil}
\addplot[black,mark=triangle,  mark options={solid}] coordinates {
(1,34629)(2,40524)(3,32741)(4,38869)(5,35222)(6,66634)(7,37901)(8,59610)(9,53793)(10,26902)(11,42503)(12,40646)
};
 \label{diez}
\addplot[black,mark=o,  mark options={solid}] coordinates {
(1,32077)(2,24030)(3,25522)(4,16195)(5,24189)(6,36450)(7,16312)(8,24143)(9,26803)(10,16368)(11,23915)(12,27213)
};
 \label{veinte}
\addplot[black,mark=ball,  mark options={solid}] coordinates {
(1,29596)(2,23883)(3,25543)(4,16304)(5,24008)(6,25408)(7,16174)(8,23877)(9,27046)(10,16400)(11,23992)(12,27124)
};
 \label{cincuenta}
\addplot[black,mark=diamond,  mark options={solid}] coordinates {
(1,30223)(2,23991)(3,25466)(4,16235)(5,23961)(6,25350)(7,16194)(8,23690)(9,27032)(10,16214)(11,23829)(12,27109)
};
 \label{cien}
\addplot[black,mark=otimes,  mark options={solid}] coordinates {
(1,138176)(2,134928)(3,431718)(4,234437)(5,231089)(6,442281)(7,326023)(8,349539)(9,343554)(10,435238)(11,440403)(12,455199)
};
 \label{quinientos}
%%%%%%%%%%%%%%%%%%%%%%%
    %View no keys!!!
%%%%%%%%%%%%%%%%%%%%%%%

\end{axis}
\end{tikzpicture}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& 

	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
\\	
\begin{minipage}{.90\textwidth}
	\centering
		\footnotesize{
			\ref{mil} $\sigma_{1.000}$~~~ 
			\ref{diez} $\sigma_{10.000}$ ~~~
			\ref{veinte} $\sigma_{20.000}$~~~
			\ref{cincuenta} $\sigma_{50.000}$~~~
			\ref{cien} $\sigma_{100.000}$ ~~~
			\ref{quinientos} $\sigma_{500.000}$ ~~~
			}
\end{minipage}
\end{tabular}

\caption{Full summary}
\label{fig:general-JUcc-UJnc-2URI}	
\end{figure*}




}



























\ignore{





\begin{figure*}[bth]
	
	\begin{tabular}{c}
	
	\begin{tabular}{cc}
		\begin{minipage}{.30\textwidth}
		\begin{tikzpicture}
		\pgfplotsset{every axis/.append style={
			font=\footnotesize,
			semithick,
			tick style={thick}}}
			% FishMark - Results
		    \begin{axis}[
				title= Postgres Pumped Str,
	    			height=7cm,
				width=14cm,
				xtick={0,1,2,3,4,5,6,7,8,9,10,11,12},
				xticklabels={0,1,2,3,4,5,6,7,8,9,10,11,12},
		        	grid=major,
				ymode=log,
				% legend to name=benchmarkset,
				legend columns=-1
		    ]
%%%%%%%%%%%%%%%%%%%%%%%    
   	     %JOINS !!
%%%%%%%%%%%%%%%%%%%%%%%
\addplot[black,mark=square,  mark options={solid}] coordinates {
(1,40485)(2,32613)(3,56302)(4,42680)(5,44615)(6,59520)(7,39019)(8,45313)(9,52960)(10,46501)(11,44107)(12,53877)
};
 \label{mil}
\addplot[black,mark=triangle,  mark options={solid}] coordinates {
(1,47018)(2,44276)(3,46710)(4,39247)(5,36732)(6,57450)(7,44652)(8,38786)(9,42775)(10,33730)(11,47297)(12,44032)
};
 \label{diez}
\addplot[black,mark=o,  mark options={solid}] coordinates {
(1,21600)(2,16510)(3,25270)(4,15762)(5,15837)(6,41981)(7,25490)(8,16243)(9,25038)(10,16069)(11,16155)(12,25048)
};
 \label{veinte}
\addplot[black,mark=ball,  mark options={solid}] coordinates {
(1,16065)(2,16044)(3,25376)(4,16007)(5,15943)(6,27218)(7,16220)(8,16302)(9,25077)(10,16206)(11,16174)(12,25210)
};
 \label{cincuenta}
\addplot[black,mark=diamond,  mark options={solid}] coordinates {
(1,16076)(2,15918)(3,25676)(4,77757)(5,75902)(6,181961)(7,16376)(8,16490)(9,25339)(10,16079)(11,16438)(12,25295)
};
 \label{cien}
\addplot[black,mark=otimes,  mark options={solid}] coordinates {
(1,146817)(2,149591)(3,480517)(4,260899)(5,249826)(6,483650)(7,363141)(8,352662)(9,362121)(10,468961)(11,462599)(12,495534)
};
 \label{quinientos}
%%%%%%%%%%%%%%%%%%%%%%%
    %View no keys!!!
%%%%%%%%%%%%%%%%%%%%%%%

\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=square,  mark options={solid}] coordinates {
(1,1200136)(2,1200947)(3,1201675)(4,1200158)(5,1200940)(6,1201615)(7,1200076)(8,1200894)(9,1201560)(10,412618)(11,482441)(12,580467)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=triangle,  mark options={solid}] coordinates {
(1,1200008)(2,1201030)(3,1201682)(4,1200015)(5,1200948)(6,1201581)(7,1200048)(8,1200829)(9,1201656)(10,359014)(11,481491)(12,580147)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=o,  mark options={solid}] coordinates {
(1,1200008)(2,1200864)(3,1201751)(4,1200020)(5,1200939)(6,1201630)(7,1200045)(8,1200880)(9,1201613)(10,354305)(11,488982)(12,578600)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=ball,  mark options={solid}] coordinates {
(1,1200007)(2,1200905)(3,1201743)(4,1200009)(5,1200967)(6,1201542)(7,1200009)(8,1200893)(9,1201647)(10,359527)(11,497104)(12,593896)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=diamond,  mark options={solid}] coordinates {
(1,1200007)(2,1200805)(3,1201749)(4,1200011)(5,1200950)(6,1201493)(7,1200005)(8,1200979)(9,1201438)(10,368976)(11,510998)(12,608056)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=otimes,  mark options={solid}] coordinates {
(1,603523)(2,926692)(3,1200022)(4,668177)(5,1081981)(6,1204434)(7,1200006)(8,1200862)(9,1201613)(10,396533)(11,563917)(12,680905)

};
\end{axis}
\end{tikzpicture}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& 

	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
\\	
\begin{minipage}{.90\textwidth}
	\centering
		\footnotesize{
			\ref{mil} $\sigma_{1.000}$~~~ 
			\ref{diez} $\sigma_{10.000}$ ~~~
			\ref{veinte} $\sigma_{20.000}$~~~
			\ref{cincuenta} $\sigma_{50.000}$~~~
			\ref{cien} $\sigma_{100.000}$ ~~~
			\ref{quinientos} $\sigma_{500.000}$ ~~~
			}
\end{minipage}
\end{tabular}

\caption{Full summary}
\label{fig:general-JUcc-UJnc-2URI}	
\end{figure*}










\begin{figure*}[htb]
\footnotesize
\center
%
\[
\begin{array}{lllllllll}
Queries &  1 SPARQL Joins  & 2 SPARQL Joins & 3 SPARQL Joins &  1 V S. Joins  & 2 V S. Joins & 3 V S. Joins & \# Results \\	
%
1 SQL Join\\
q_{1} & 40485 & 32613 & 56302 & 214469 & 361966 & 515601 \\
q_{2} &47018 & 44276 & 46710  & 207187 & 365883 & 514732\\
q_{3} &21600 & 16510 & 25270 & 206462 & 366102 & 512519\\
q_{4} &16065 & 16044 & 25376 &202872 & 364345 & 518088 \\
q_{5} &16076 & 15918 & 25676 & 203960 & 360827 & 508873\\
q_{6} &146817 & 149591 & 480517 & 272552 & 469315 & 665422 \\
2 SQL Join\\
q_{7} &42680 & 44615 & 59520 & 205144 & 350249 & 507112\\
q_{8} &39247 & 36732 & 57450 & 206213 & 354194 & 503774\\
q_{9} &15762 & 15837 & 41981 & 206230 & 352414 & 507075\\
q_{10} &16007 & 15943 & 27218 & 207280 & 355663 & 512996\\
q_{11} &77757 & 75902 & 181961 & 211188 & 357269 & 503463\\
q_{12} &260899 & 249826 & 483650 & 272027 & 471609 & 666856\\
3 SQL Join\\
q_{13} &39019 & 45313 & 52960 & 232461 & 385723 & 543077\\
q_{14} &44652 & 38786 & 42775 & 234350 & 390995 & 532887\\
q_{15} &25490 & 16243 & 25038 & 232780 & 389376 & 541941\\
q_{16} &16220 & 16302 & 25077 & 237110 & 390653 & 541513 \\
q_{17} &16376 & 16490 & 25339 & 236604 & 394173 & 539756\\
q_{18} &363141 & 352662 & 362121 & 293071 & 494297 & 690269\\
4 SQL Join\\
q_{19} &46501 & 44107 & 53877 & 308880 & 456907 & 614897\\
q_{20} &33730 & 47297 & 44032 & 311068 & 455669 & 607153\\
q_{21} &16069 & 16155 & 25048 & 307550 & 457892 & 612118\\
q_{22} &16206 & 16174 & 25210 & 304073 & 451282 & 604200\\
q_{23} &16079 & 16438 & 25295 & 302755 & 460672 & 608041\\
q_{24} &468961 & 462599 & 495534 & 356619 & 556889 & 754702 \\
\end{array}
\]
\caption{ Results String Joins vs Views - PostgresSQL Pumped }
\end{figure*}
}


























\begin{minipage}{.30\textwidth}
\begin{tikzpicture}
\pgfplotsset{every axis/.append style={
			font=\footnotesize,
			semithick,
			tick style={thick}}}
			% FishMark - Results
		    \begin{axis}[
				title= Postgres  100M Str. Keys (log scale),
	    			height=6cm,
				width=10cm,
				xtick={0,1,2,3,4,5,6,7,8,9,10,11,12},
				xticklabels={0,1,2,3,4,5,6,7,8,9,10,11,12},
				ytick={10000,100000,1000000,10000000,100000000},
		        	grid=major,
				ymode=log,
				% legend to name=benchmarkset,
				legend columns=-1
		    ]
%%%%%%%%%%%%%%%%%%%%%%%    
   	     %JOINS !!
%%%%%%%%%%%%%%%%%%%%%%%
\addplot[black,mark=square,  mark options={solid}] coordinates {
(1,40680)(2,21399)(3,29716)(4,68438)(5,69425)(6,74578)(7,64491)(8,66527)(9,69770)(10,63787)(11,63689)(12,68142)

};
 \label{mil}
\addplot[black,mark=triangle,  mark options={solid}] coordinates {
(1,21053)(2,21228)(3,29590)(4,67848)(5,70111)(6,74342)(7,65768)(8,67512)(9,70360)(10,64552)(11,63469)(12,66814)

};
 \label{diez}
\addplot[black,mark=o,  mark options={solid}] coordinates {
(1,21034)(2,21277)(3,29659)(4,67112)(5,69398)(6,75141)(7,64536)(8,67012)(9,70621)(10,63956)(11,63356)(12,67608)

};
 \label{veinte}
\addplot[black,mark=ball,  mark options={solid}] coordinates {
(1,21108)(2,20514)(3,29673)(4,68995)(5,69300)(6,75639)(7,64896)(8,67665)(9,71342)(10,64216)(11,64201)(12,67984)

};
 \label{cincuenta}
\addplot[black,mark=diamond,  mark options={solid}] coordinates {
(1,21269)(2,20658)(3,30627)(4,67926)(5,71610)(6,75953)(7,64100)(8,67916)(9,70697)(10,63535)(11,64153)(12,70415)
};
 \label{cien}
\addplot[black,mark=otimes,  mark options={solid}] coordinates {
(1,24056)(2,23077)(3,33547)(4,70502)(5,73307)(6,80208)(7,148820)(8,151626)(9,157293)(10,149074)(11,151063)(12,155835)

};
 \label{quinientos}
%%%%%%%%%%%%%%%%%%%%%%%
    %View no keys!!!
%%%%%%%%%%%%%%%%%%%%%%%

\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=square,  mark options={solid}] coordinates {
(1,1200004)(2,1200864)(3,1201598)(4,1200008)(5,1200979)(6,1201628)(7,1200006)(8,1200962)(9,1201577)(10,327793)(11,483859)(12,637656)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=triangle,  mark options={solid}] coordinates {
(1,1200005)(2,1201025)(3,1201619)(4,1200004)(5,1200823)(6,1201679)(7,1200004)(8,1200920)(9,1201595)(10,319908)(11,481577)(12,637879)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=o,  mark options={solid}] coordinates {
(1,1200005)(2,1200999)(3,1201773)(4,1200004)(5,1200864)(6,1201628)(7,1200020)(8,1200880)(9,1201625)(10,327109)(11,482407)(12,641166)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=ball,  mark options={solid}] coordinates {
(1,1200004)(2,1201017)(3,1201750)(4,1200004)(5,1200879)(6,1201742)(7,1200003)(8,1200898)(9,1201564)(10,323762)(11,490466)(12,652036)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=diamond,  mark options={solid}] coordinates {
(1,1200004)(2,1200776)(3,1201727)(4,1200003)(5,1200939)(6,1201658)(7,1200008)(8,1200911)(9,1201607)(10,331205)(11,505615)(12,667839)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=otimes,  mark options={solid}] coordinates {
(1,532694)(2,920665)(3,1200013)(4,588098)(5,1087825)(6,1204842)(7,1200006)(8,1200903)(9,1201628)(10,355050)(11,546973)(12,743397)

};

%%%%%%%%%%%%%%%%%%%%%%%
    %View Tuned keys!!!
%%%%%%%%%%%%%%%%%%%%%%%



\addplot[black,densely dotted,mark=square,  mark options={solid}] coordinates {
(1,154431)(2,158150)(3,158569)(4,197129)(5,195267)(6,199008)(7,254345)(8,250737)(9,253343)(10,169087)(11,166836)(12,168196)
};

\addplot[black,densely dotted,mark=triangle,  mark options={solid}] coordinates {
(1,154369)(2,156015)(3,157581)(4,196632)(5,198836)(6,201255)(7,251874)(8,252234)(9,254502)(10,165453)(11,166968)(12,169425)
};

\addplot[black,densely dotted,mark=o,  mark options={solid}] coordinates {
(1,155608)(2,157952)(3,157628)(4,195819)(5,200102)(6,201829)(7,256532)(8,250505)(9,252045)(10,168054)(11,168612)(12,170006)
};

\addplot[black,densely dotted,mark=ball,  mark options={solid}] coordinates {
(1,155829)(2,158690)(3,159180)(4,197900)(5,199376)(6,198640)(7,251399)(8,254978)(9,254437)(10,170905)(11,168260)(12,171479)
};

\addplot[black,densely dotted,mark=diamond,  mark options={solid}] coordinates {
(1,154627)(2,157907)(3,158205)(4,197702)(5,200828)(6,200971)(7,251931)(8,254663)(9,256738)(10,167334)(11,170532)(12,169671)
};

\addplot[black,densely dotted,mark=otimes,  mark options={solid}] coordinates {
(1,155053)(2,159548)(3,160992)(4,197929)(5,199820)(6,198866)(7,256193)(8,254801)(9,258106)(10,169054)(11,172915)(12,171791)
};


\end{axis}
\end{tikzpicture}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




	
\begin{minipage}{.90\textwidth}
	\centering
		\footnotesize{
			\ref{mil} $\sigma_{100}$~~~ 
			\ref{diez} $\sigma_{500}$ ~~~
			\ref{veinte} $\sigma_{1.000}$\\
			\ref{cincuenta} $\sigma_{5.000}$~~~
			\ref{cien} $\sigma_{10.000}$ ~~~
			\ref{quinientos} $\sigma_{100.000}$ ~~~
			}
\end{minipage}


\caption{Full summary}
\label{fig:postgresInt100M}	
\end{figure*}










%\begin{figure*}[bth]
\begin{figure*}
		\begin{minipage}{.30\textwidth}
		\begin{tikzpicture}
		\pgfplotsset{every axis/.append style={
			font=\footnotesize,
			semithick,
			tick style={thick}}}
			% FishMark - Results
		    \begin{axis}[
				title= Postgres 100M Int. Keys (log scale),
	    			height=6cm,
				width=10cm,
				xtick={0,1,2,3,4,5,6,7,8,9,10,11,12},
				xticklabels={0,1,2,3,4,5,6,7,8,9,10,11,12},
				ytick={10000,100000,1000000,10000000,100000000},
		        	grid=major,
				ymode=log,
				% legend to name=benchmarkset,
				legend columns=1
		    ]
%%%%%%%%%%%%%%%%%%%%%%%    
   	     %JOINS !!
%%%%%%%%%%%%%%%%%%%%%%%
\addplot[black,mark=square,  mark options={solid}] coordinates {
(1,16050)(2,33857)(3,28549)
(4,19318)(5,26602)(6,29124)
(7,23136)(8,25402)(9,28495)
(10,29457)(11,35878)(12,32541)
};
 \label{mil}
\addplot[black,mark=triangle,  mark options={solid}] coordinates {
(1,15801)(2,23662)(3,26400)
(4,15733)(5,23357)(6,26630)
(7,15323)(8,23280)(9,26473)
(10,15738)(11,23830)(12,26654)
};
 \label{diez}
\addplot[black,mark=o,  mark options={solid}] coordinates {
(1,15744)(2,23543)(3,26364)
(4,15699)(5,23255)(6,26613)
(7,15371)(8,23663)(9,26627)
(10,15736)(11,23751)(12,26903)
};
 \label{veinte}
\addplot[black,mark=ball,  mark options={solid}] coordinates {
(1,15797)(2,23743)(3,26546)
(4,15828)(5,23424)(6,26811)
(7,15445)(8,23761)(9,26556)
(10,15861)(11,23851)(12,26753)
};

%%%%%%%%%%%%%%%%%%%%%%%
    %View no keys!!!
%%%%%%%%%%%%%%%%%%%%%%%
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=square,  mark options={solid}] coordinates {
(1,940016)(2,1200254)(3,1200429)(4,1122649)(5,1200230)(6,1200406)(7,1200032)(8,1200226)(9,1200356)(10,1200025)(11,1200014)(12,1200016)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=triangle,  mark options={solid}] coordinates {
(1,1200017)(2,1200270)(3,1200386)(4,1200026)(5,1200241)(6,1200386)(7,1200018)(8,1200225)(9,1200371)(10,1200007)(11,1200016)(12,1200009)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=o,  mark options={solid}] coordinates {
(1,1200008)(2,1200266)(3,1200395)(4,1200019)(5,1200249)(6,1200379)(7,1200012)(8,1200265)(9,1200388)(10,1194633)(11,1200060)(12,1200008)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=ball,  mark options={solid}] coordinates {
(1,1200009)(2,1200310)(3,1200438)(4,1200013)(5,1200199)(6,1200405)(7,1200010)(8,1200228)(9,1200384)(10,1169850)(11,1200015)(12,1200007)

};

%%%%%%%%%%%%%%%%%%%%%%%
    %View Tuned keys!!!
%%%%%%%%%%%%%%%%%%%%%%%
\addplot[black,densely dotted,mark=square,  mark options={solid}] coordinates {
(1,48947)(2,66852)(3,77979)(4,199750)(5,198910)(6,199721)(7,284036)(8,284189)(9,286047)(10,658571)(11,655541)(12,661470)
};

\addplot[black,densely dotted,mark=triangle,  mark options={solid}] coordinates {
(1,43298)(2,43774)(3,46325)(4,199491)(5,199003)(6,200654)(7,280808)(8,283823)(9,283746)(10,659654)(11,655298)(12,661997)
};

\addplot[black,densely dotted,mark=o,  mark options={solid}] coordinates {
(1,43359)(2,43482)(3,45898)(4,200155)(5,198885)(6,199745)(7,283582)(8,287859)(9,285676)(10,660197)(11,656282)(12,659368)
};

\addplot[black,densely dotted,mark=ball,  mark options={solid}] coordinates {
(1,43727)(2,43480)(3,46349)(4,199921)(5,200364)(6,201746)(7,286378)(8,284764)(9,284998)(10,660355)(11,660309)(12,660880)
};

\end{axis}
\end{tikzpicture}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{minipage}{.30\textwidth}
\begin{tikzpicture}
\pgfplotsset{every axis/.append style={
			font=\footnotesize,
			semithick,
			tick style={thick}}}
			% FishMark - Results
		    \begin{axis}[
				title= Postgres  100M Str. Keys (log scale),
	    			height=6cm,
				width=10cm,
				xtick={0,1,2,3,4,5,6,7,8,9,10,11,12},
				xticklabels={0,1,2,3,4,5,6,7,8,9,10,11,12},
				ytick={10000,100000,1000000,10000000,100000000},
		        	grid=major,
				ymode=log,
				% legend to name=benchmarkset,
				legend columns=-1
		    ]
%%%%%%%%%%%%%%%%%%%%%%%    
   	     %JOINS !!
%%%%%%%%%%%%%%%%%%%%%%%
\addplot[black,mark=square,  mark options={solid}] coordinates {
(1,40680)(2,21399)(3,29716)(4,68438)(5,69425)(6,74578)(7,64491)(8,66527)(9,69770)(10,63787)(11,63689)(12,68142)

};
 \label{mil}
\addplot[black,mark=triangle,  mark options={solid}] coordinates {
(1,21053)(2,21228)(3,29590)(4,67848)(5,70111)(6,74342)(7,65768)(8,67512)(9,70360)(10,64552)(11,63469)(12,66814)

};
 \label{diez}
\addplot[black,mark=o,  mark options={solid}] coordinates {
(1,21034)(2,21277)(3,29659)(4,67112)(5,69398)(6,75141)(7,64536)(8,67012)(9,70621)(10,63956)(11,63356)(12,67608)

};
 \label{veinte}
\addplot[black,mark=ball,  mark options={solid}] coordinates {
(1,21108)(2,20514)(3,29673)(4,68995)(5,69300)(6,75639)(7,64896)(8,67665)(9,71342)(10,64216)(11,64201)(12,67984)

};
 \label{cincuenta}
\addplot[black,mark=diamond,  mark options={solid}] coordinates {
(1,21269)(2,20658)(3,30627)(4,67926)(5,71610)(6,75953)(7,64100)(8,67916)(9,70697)(10,63535)(11,64153)(12,70415)
};
 \label{cien}
\addplot[black,mark=otimes,  mark options={solid}] coordinates {
(1,24056)(2,23077)(3,33547)(4,70502)(5,73307)(6,80208)(7,148820)(8,151626)(9,157293)(10,149074)(11,151063)(12,155835)

};
 \label{quinientos}
%%%%%%%%%%%%%%%%%%%%%%%
    %View no keys!!!
%%%%%%%%%%%%%%%%%%%%%%%

\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=square,  mark options={solid}] coordinates {
(1,1200004)(2,1200864)(3,1201598)(4,1200008)(5,1200979)(6,1201628)(7,1200006)(8,1200962)(9,1201577)(10,327793)(11,483859)(12,637656)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=triangle,  mark options={solid}] coordinates {
(1,1200005)(2,1201025)(3,1201619)(4,1200004)(5,1200823)(6,1201679)(7,1200004)(8,1200920)(9,1201595)(10,319908)(11,481577)(12,637879)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=o,  mark options={solid}] coordinates {
(1,1200005)(2,1200999)(3,1201773)(4,1200004)(5,1200864)(6,1201628)(7,1200020)(8,1200880)(9,1201625)(10,327109)(11,482407)(12,641166)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=ball,  mark options={solid}] coordinates {
(1,1200004)(2,1201017)(3,1201750)(4,1200004)(5,1200879)(6,1201742)(7,1200003)(8,1200898)(9,1201564)(10,323762)(11,490466)(12,652036)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=diamond,  mark options={solid}] coordinates {
(1,1200004)(2,1200776)(3,1201727)(4,1200003)(5,1200939)(6,1201658)(7,1200008)(8,1200911)(9,1201607)(10,331205)(11,505615)(12,667839)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=otimes,  mark options={solid}] coordinates {
(1,532694)(2,920665)(3,1200013)(4,588098)(5,1087825)(6,1204842)(7,1200006)(8,1200903)(9,1201628)(10,355050)(11,546973)(12,743397)

};

%%%%%%%%%%%%%%%%%%%%%%%
    %View Tuned keys!!!
%%%%%%%%%%%%%%%%%%%%%%%



\addplot[black,densely dotted,mark=square,  mark options={solid}] coordinates {
(1,154431)(2,158150)(3,158569)(4,197129)(5,195267)(6,199008)(7,254345)(8,250737)(9,253343)(10,169087)(11,166836)(12,168196)
};

\addplot[black,densely dotted,mark=triangle,  mark options={solid}] coordinates {
(1,154369)(2,156015)(3,157581)(4,196632)(5,198836)(6,201255)(7,251874)(8,252234)(9,254502)(10,165453)(11,166968)(12,169425)
};

\addplot[black,densely dotted,mark=o,  mark options={solid}] coordinates {
(1,155608)(2,157952)(3,157628)(4,195819)(5,200102)(6,201829)(7,256532)(8,250505)(9,252045)(10,168054)(11,168612)(12,170006)
};

\addplot[black,densely dotted,mark=ball,  mark options={solid}] coordinates {
(1,155829)(2,158690)(3,159180)(4,197900)(5,199376)(6,198640)(7,251399)(8,254978)(9,254437)(10,170905)(11,168260)(12,171479)
};

\addplot[black,densely dotted,mark=diamond,  mark options={solid}] coordinates {
(1,154627)(2,157907)(3,158205)(4,197702)(5,200828)(6,200971)(7,251931)(8,254663)(9,256738)(10,167334)(11,170532)(12,169671)
};

\addplot[black,densely dotted,mark=otimes,  mark options={solid}] coordinates {
(1,155053)(2,159548)(3,160992)(4,197929)(5,199820)(6,198866)(7,256193)(8,254801)(9,258106)(10,169054)(11,172915)(12,171791)
};


\end{axis}
\end{tikzpicture}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




	
\begin{minipage}{.90\textwidth}
	\centering
		\footnotesize{
			\ref{mil} $\sigma_{100}$~~~ 
			\ref{diez} $\sigma_{500}$ ~~~
			\ref{veinte} $\sigma_{1.000}$\\
			\ref{cincuenta} $\sigma_{5.000}$~~~
			\ref{cien} $\sigma_{10.000}$ ~~~
			\ref{quinientos} $\sigma_{100.000}$ ~~~
			}
\end{minipage}


\caption{Full summary}
\label{fig:postgresInt100M}	
\end{figure*}
































\almargen{we need to re-do these experiments-commented}

\ignore{
\begin{figure*}[bth]
	
	\begin{tabular}{c}
	
	\begin{tabular}{cc}
		\begin{minipage}{.30\textwidth}
		\begin{tikzpicture}
		\pgfplotsset{every axis/.append style={
			font=\footnotesize,
			semithick,
			tick style={thick}}}
			% FishMark - Results
		    \begin{axis}[
				title= Postgres Pumped Int,
	    			height=7cm,
				width=14cm,
				xtick={0,1,2,3,4,5,6,7,8,9,10,11,12},
				xticklabels={0,1,2,3,4,5,6,7,8,9,10,11,12},
		        	grid=major,
				ymode=log,
				% legend to name=benchmarkset,
				legend columns=-1
		    ]
%%%%%%%%%%%%%%%%%%%%%%%    
   	     %JOINS !!
%%%%%%%%%%%%%%%%%%%%%%%
\addplot[black,mark=square,  mark options={solid}] coordinates {
(1,36463)(2,56721)(3,63524)(4,39960)(5,50929)(6,62401)(7,41697)(8,59913)(9,61102)(10,46885)(11,49938)(12,52916)
};
 \label{mil}
\addplot[black,mark=triangle,  mark options={solid}] coordinates {
(1,34629)(2,40524)(3,32741)(4,38869)(5,35222)(6,66634)(7,37901)(8,59610)(9,53793)(10,26902)(11,42503)(12,40646)
};
 \label{diez}
\addplot[black,mark=o,  mark options={solid}] coordinates {
(1,32077)(2,24030)(3,25522)(4,16195)(5,24189)(6,36450)(7,16312)(8,24143)(9,26803)(10,16368)(11,23915)(12,27213)
};
 \label{veinte}
\addplot[black,mark=ball,  mark options={solid}] coordinates {
(1,29596)(2,23883)(3,25543)(4,16304)(5,24008)(6,25408)(7,16174)(8,23877)(9,27046)(10,16400)(11,23992)(12,27124)
};
 \label{cincuenta}
\addplot[black,mark=diamond,  mark options={solid}] coordinates {
(1,30223)(2,23991)(3,25466)(4,16235)(5,23961)(6,25350)(7,16194)(8,23690)(9,27032)(10,16214)(11,23829)(12,27109)
};
 \label{cien}
\addplot[black,mark=otimes,  mark options={solid}] coordinates {
(1,138176)(2,134928)(3,431718)(4,234437)(5,231089)(6,442281)(7,326023)(8,349539)(9,343554)(10,435238)(11,440403)(12,455199)
};
 \label{quinientos}
%%%%%%%%%%%%%%%%%%%%%%%
    %View no keys!!!
%%%%%%%%%%%%%%%%%%%%%%%

\end{axis}
\end{tikzpicture}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& 

	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
\\	
\begin{minipage}{.90\textwidth}
	\centering
		\footnotesize{
			\ref{mil} $\sigma_{1.000}$~~~ 
			\ref{diez} $\sigma_{10.000}$ ~~~
			\ref{veinte} $\sigma_{20.000}$~~~
			\ref{cincuenta} $\sigma_{50.000}$~~~
			\ref{cien} $\sigma_{100.000}$ ~~~
			\ref{quinientos} $\sigma_{500.000}$ ~~~
			}
\end{minipage}
\end{tabular}

\caption{Full summary}
\label{fig:general-JUcc-UJnc-2URI}	
\end{figure*}




}



























\ignore{





\begin{figure*}[bth]
	
	\begin{tabular}{c}
	
	\begin{tabular}{cc}
		\begin{minipage}{.30\textwidth}
		\begin{tikzpicture}
		\pgfplotsset{every axis/.append style={
			font=\footnotesize,
			semithick,
			tick style={thick}}}
			% FishMark - Results
		    \begin{axis}[
				title= Postgres Pumped Str,
	    			height=7cm,
				width=14cm,
				xtick={0,1,2,3,4,5,6,7,8,9,10,11,12},
				xticklabels={0,1,2,3,4,5,6,7,8,9,10,11,12},
		        	grid=major,
				ymode=log,
				% legend to name=benchmarkset,
				legend columns=-1
		    ]
%%%%%%%%%%%%%%%%%%%%%%%    
   	     %JOINS !!
%%%%%%%%%%%%%%%%%%%%%%%
\addplot[black,mark=square,  mark options={solid}] coordinates {
(1,40485)(2,32613)(3,56302)(4,42680)(5,44615)(6,59520)(7,39019)(8,45313)(9,52960)(10,46501)(11,44107)(12,53877)
};
 \label{mil}
\addplot[black,mark=triangle,  mark options={solid}] coordinates {
(1,47018)(2,44276)(3,46710)(4,39247)(5,36732)(6,57450)(7,44652)(8,38786)(9,42775)(10,33730)(11,47297)(12,44032)
};
 \label{diez}
\addplot[black,mark=o,  mark options={solid}] coordinates {
(1,21600)(2,16510)(3,25270)(4,15762)(5,15837)(6,41981)(7,25490)(8,16243)(9,25038)(10,16069)(11,16155)(12,25048)
};
 \label{veinte}
\addplot[black,mark=ball,  mark options={solid}] coordinates {
(1,16065)(2,16044)(3,25376)(4,16007)(5,15943)(6,27218)(7,16220)(8,16302)(9,25077)(10,16206)(11,16174)(12,25210)
};
 \label{cincuenta}
\addplot[black,mark=diamond,  mark options={solid}] coordinates {
(1,16076)(2,15918)(3,25676)(4,77757)(5,75902)(6,181961)(7,16376)(8,16490)(9,25339)(10,16079)(11,16438)(12,25295)
};
 \label{cien}
\addplot[black,mark=otimes,  mark options={solid}] coordinates {
(1,146817)(2,149591)(3,480517)(4,260899)(5,249826)(6,483650)(7,363141)(8,352662)(9,362121)(10,468961)(11,462599)(12,495534)
};
 \label{quinientos}
%%%%%%%%%%%%%%%%%%%%%%%
    %View no keys!!!
%%%%%%%%%%%%%%%%%%%%%%%

\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=square,  mark options={solid}] coordinates {
(1,1200136)(2,1200947)(3,1201675)(4,1200158)(5,1200940)(6,1201615)(7,1200076)(8,1200894)(9,1201560)(10,412618)(11,482441)(12,580467)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=triangle,  mark options={solid}] coordinates {
(1,1200008)(2,1201030)(3,1201682)(4,1200015)(5,1200948)(6,1201581)(7,1200048)(8,1200829)(9,1201656)(10,359014)(11,481491)(12,580147)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=o,  mark options={solid}] coordinates {
(1,1200008)(2,1200864)(3,1201751)(4,1200020)(5,1200939)(6,1201630)(7,1200045)(8,1200880)(9,1201613)(10,354305)(11,488982)(12,578600)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=ball,  mark options={solid}] coordinates {
(1,1200007)(2,1200905)(3,1201743)(4,1200009)(5,1200967)(6,1201542)(7,1200009)(8,1200893)(9,1201647)(10,359527)(11,497104)(12,593896)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=diamond,  mark options={solid}] coordinates {
(1,1200007)(2,1200805)(3,1201749)(4,1200011)(5,1200950)(6,1201493)(7,1200005)(8,1200979)(9,1201438)(10,368976)(11,510998)(12,608056)

};
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=otimes,  mark options={solid}] coordinates {
(1,603523)(2,926692)(3,1200022)(4,668177)(5,1081981)(6,1204434)(7,1200006)(8,1200862)(9,1201613)(10,396533)(11,563917)(12,680905)

};
\end{axis}
\end{tikzpicture}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& 

	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
\\	
\begin{minipage}{.90\textwidth}
	\centering
		\footnotesize{
			\ref{mil} $\sigma_{1.000}$~~~ 
			\ref{diez} $\sigma_{10.000}$ ~~~
			\ref{veinte} $\sigma_{20.000}$~~~
			\ref{cincuenta} $\sigma_{50.000}$~~~
			\ref{cien} $\sigma_{100.000}$ ~~~
			\ref{quinientos} $\sigma_{500.000}$ ~~~
			}
\end{minipage}
\end{tabular}

\caption{Full summary}
\label{fig:general-JUcc-UJnc-2URI}	
\end{figure*}










\begin{figure*}[htb]
\footnotesize
\center
%
\[
\begin{array}{lllllllll}
Queries &  1 SPARQL Joins  & 2 SPARQL Joins & 3 SPARQL Joins &  1 V S. Joins  & 2 V S. Joins & 3 V S. Joins & \# Results \\	
%
1 SQL Join\\
q_{1} & 40485 & 32613 & 56302 & 214469 & 361966 & 515601 \\
q_{2} &47018 & 44276 & 46710  & 207187 & 365883 & 514732\\
q_{3} &21600 & 16510 & 25270 & 206462 & 366102 & 512519\\
q_{4} &16065 & 16044 & 25376 &202872 & 364345 & 518088 \\
q_{5} &16076 & 15918 & 25676 & 203960 & 360827 & 508873\\
q_{6} &146817 & 149591 & 480517 & 272552 & 469315 & 665422 \\
2 SQL Join\\
q_{7} &42680 & 44615 & 59520 & 205144 & 350249 & 507112\\
q_{8} &39247 & 36732 & 57450 & 206213 & 354194 & 503774\\
q_{9} &15762 & 15837 & 41981 & 206230 & 352414 & 507075\\
q_{10} &16007 & 15943 & 27218 & 207280 & 355663 & 512996\\
q_{11} &77757 & 75902 & 181961 & 211188 & 357269 & 503463\\
q_{12} &260899 & 249826 & 483650 & 272027 & 471609 & 666856\\
3 SQL Join\\
q_{13} &39019 & 45313 & 52960 & 232461 & 385723 & 543077\\
q_{14} &44652 & 38786 & 42775 & 234350 & 390995 & 532887\\
q_{15} &25490 & 16243 & 25038 & 232780 & 389376 & 541941\\
q_{16} &16220 & 16302 & 25077 & 237110 & 390653 & 541513 \\
q_{17} &16376 & 16490 & 25339 & 236604 & 394173 & 539756\\
q_{18} &363141 & 352662 & 362121 & 293071 & 494297 & 690269\\
4 SQL Join\\
q_{19} &46501 & 44107 & 53877 & 308880 & 456907 & 614897\\
q_{20} &33730 & 47297 & 44032 & 311068 & 455669 & 607153\\
q_{21} &16069 & 16155 & 25048 & 307550 & 457892 & 612118\\
q_{22} &16206 & 16174 & 25210 & 304073 & 451282 & 604200\\
q_{23} &16079 & 16438 & 25295 & 302755 & 460672 & 608041\\
q_{24} &468961 & 462599 & 495534 & 356619 & 556889 & 754702 \\
\end{array}
\]
\caption{ Results String Joins vs Views - PostgresSQL Pumped }
\end{figure*}
}


\subsection{Experiments with SMALL POSTGRES}
\input{graphs/graph-smallpostgres-int.tex}
\input{graphs/graph-smallpostgres-str.tex}


==> graphs/cte/npd/query_bars.tex <==
  \begin{tabular}{c}
    \begin{tabular}{c}
      \begin{minipage}{.5\textwidth}
        %\centering
        \hspace{.0\textwidth}
	\begin{tikzpicture}
	  \pgfplotsset{every axis/.append style={
	      font=\footnotesize,
	      semithick,
	      tick style={thick}}}
	  % FishMark - Results
          \begin{axis}[
              name=bottom axis,
	      ybar=0pt,
              bar width=0.1cm,
	      height=2cm,
	      width=6cm,
      	      xtick={1,2,3,4,5,6},
      	      xticklabels={$q_{6}^p$,$q_{6}^{d}$,$q_{11}^p$,$q_{11}^{d}$,$q_{12}^p$,$q_{12}^{d}$},
	      ytick=\empty,
              yticklabels=\empty,
	      grid=major,
	      legend columns=-1,
              ymin=0, 
	      ymax=10000,
              %ymode=log,
              axis x line*=bottom
	    ]

            \addplot[fill=blue!60] coordinates {
              (1,10000) % q-06-untuned.sql
              (3,10000) % q-11-untuned.sql
              (5,10000) % q-12-untuned.sql

              (2,10000) % q-06-untuned db2
              (4,10000) % q-11-untuned db2
              (6,10000) % q-12-untuned db2
	    };
	    %\label{untuned}
	    \addplot[draw=black, pattern color = black, pattern = horizontal lines] coordinates {
              (1,10000) % q-06-tuned-selfJoin.sql
              (3,10000) % q-11-tuned-selfJoin.sql
              (5,10000) % q-12-tuned-selfJoin.sql

              (2,10000) % q-06-tuned-selfjoin.sql db2
              (4,10000) % q-11-tuned-self db2
              (6,10000) % q-12-tuned-self db2
	    };
            %\label{tuned-self}
            \addplot[draw=red, pattern color = red, pattern = north west lines] coordinates {
              (1,10000) % q-06-tuned-full.sql
              (3,10000) % q-11-tuned-full.sql
              (5,10000) % q-12-tuned-full.sql

              (2,10000) % q-06-tuned-full.sql db2
              (4,10000) % q-11-tuned-full db2
              (6,10000) % q-12-tuned-full db2
              
	    };
            
          \end{axis}
	  \begin{axis}[
              at=(bottom axis.north),
              anchor=south, yshift=\pgfkeysvalueof{/tikz/axis break gap},
	      ybar=0pt,
              bar width=0.1cm,
              ylabel=Query exec. time (ms.),
	      height=4cm,
	      width=6cm,
      	      xtick={1,2,3,4,5,6},
      	      %xticklabels={$q_{6}^p$,$q_{6}^{d}$,$q_{11}^p$,$q_{11}^{d}$,$q_{12}^p$,$q_{12}^{d}$},
	      %ytick={10000,100000,1000000},
	      grid=major,
	      legend columns=-1,
              ymin=10000, 
	      ymax=1200000,
              ymode=log,
              xticklabel=\empty,
              axis x line*=top, %% remove the top line
              after end axis/.code={
                \draw (rel axis cs:0,0) +(-1mm,-1mm) -- +(1mm,1mm)
                    ++(0pt,-\pgfkeysvalueof{/tikz/axis break gap})
                    +(-1mm,-1mm) -- +(1mm,1mm)
                    (rel axis cs:1,0) +(-1mm,-1mm) -- +(1mm,1mm)
                    ++(0pt,-\pgfkeysvalueof{/tikz/axis break gap})
                    +(-1mm,-1mm) -- +(1mm,1mm);
            }
	    ]
	    
	    \addplot[fill=blue!60] coordinates {
              (1,32867) % q-06-untuned.sql
              (3,126346) % q-11-untuned.sql
              (5,525873) % q-12-untuned.sql

              (2,19788) % q-06-untuned db2
              (4,107433) % q-11-untuned db2
              (6,100370) % q-12-untuned db2
	    };
	    \label{npd-untuned}
	    \addplot[draw=black, pattern color = black, pattern = horizontal lines] coordinates {
              (1,31236) % q-06-tuned-selfJoin.sql
              (3,4327372) % q-11-tuned-selfJoin.sql
              (5,2230978) % q-12-tuned-selfJoin.sql

              (2,20060) % q-06-tuned-selfjoin.sql db2
              (4,107245) % q-11-tuned-self db2
              (6,102182) % q-12-tuned-self db2
	    };
            \label{npd-tuned-self}
            \addplot[draw=red, pattern color = red, pattern = north west lines] coordinates {
              (1,15920) % q-06-tuned-full.sql
              (3,113192) % q-11-tuned-full.sql
              (5,95301) % q-12-tuned-full.sql

              (2,12867) % q-06-tuned-full.sql db2
              (4,54369) % q-11-tuned-full db2
              (6,52148) % q-12-tuned-full db2
              
	    };
            \label{npd-tuned-full}
            
	  \end{axis}
	\end{tikzpicture}
      \end{minipage}
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \end{tabular}
    \\	
    \begin{minipage}{.5\textwidth}
      %\centering
      \hspace{.12\textwidth}
      \footnotesize{
	\ref{npd-untuned} None~~~ 
	\ref{npd-tuned-self} CTE-Self~~~
        \ref{npd-tuned-full} CTE-Full~~~
      }
    \end{minipage}
\end{tabular}





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../../main"
%%% End:


==> graphs/cte/npd/query_bars_db2.tex <==
\begin{center}
  \begin{figure}
  \begin{tabular}{c}
    \begin{tabular}{c}
      \begin{minipage}{.5\textwidth}
        %\centering
        \hspace{.13\textwidth}
	\begin{tikzpicture}
	  \pgfplotsset{every axis/.append style={
	      font=\footnotesize,
	      semithick,
	      tick style={thick}}}
	  % FishMark - Results
	  \begin{axis}[
	      ybar=0pt,
              bar width=0.1cm,
              title=\textsc{NPD},
	      height=5cm,
	      %width=9cm,
      	      xtick={1,2,3},
      	      xticklabels={$q_{6}$,$q_{11}$,$q_{12}$},
	      ytick={10,1000,10000,100000,1000000},
	      grid=major,
	      legend columns=-1,
              %ymin=1, 
	      %ymax=1000000,
              ymode=log
	    ]
	    
	    \addplot[fill=blue!60] coordinates {
              (1,19788) % q-06-untuned
              (2,107433) % q-11-untuned
              (3,100370) % q-12-untuned
	    };
	    \label{untuned}
	    \addplot[draw=black, pattern color = black, pattern = horizontal lines] coordinates {
              (1,20060) % q-06-tuned-selfjoin.sql
              (2,107245) % q-11-tuned-self
              (3,102182) % q-12-tuned-self
	    };
            \label{tuned-self}
            \addplot[draw=red, pattern color = red, pattern = north west lines] coordinates {
              (1,12867) % q-06-tuned-full.sql
              (2,54369) % q-11-tuned-full
              (3,52148) % q-12-tuned-full
	    };
            \label{tuned-full}
            
	  \end{axis}
	\end{tikzpicture}
      \end{minipage}
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \end{tabular}
    \\	
    \begin{minipage}{.5\textwidth}
      %\centering
      \hspace{.15\textwidth}
      \footnotesize{
	\ref{untuned} UNF~~~ 
	\ref{tuned-self} CTE-Self~~~
        \ref{tuned-full} CTE-Full~~~
      }
    \end{minipage}
  \end{tabular}
  
  \caption{CTE Tuning on NPD}
  \label{fig:ontopVsStardog}	
\end{figure}
\end{center}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> graphs/cte/npd_wisc_bars.tex <==
%!TEX root = ../../main.tex
\hspace{-3ex}
\begin{tabular}{ll}
            \hspace{-10ex}
            \begin{minipage}{.2\textwidth}
        %    \centering
        \hspace{-5ex}
	    \begin{tikzpicture}
      	\pgfplotsset{every axis/.append style={
      	    font=\scriptsize,
      	    semithick,
      	    tick style={thick}}}

              \begin{axis}[
                  name=bottom axis,
      	    ybar=0pt,
                  bar width=0.1cm,
      	    height=2cm,
      	    width=4cm,
            	    xtick={1,2,3,4,5,6},
            	    xticklabels={$q_{A1}^p$,$q_{A1}^d$,$q_{A4}^p$,$q_{A4}^d$},
      	    ytick=\empty,
                  yticklabels=\empty,
      	    grid=major,
      	    legend columns=-1,
                  ymin=0, 
      	    ymax=10000,
                  %ymode=log,
                  axis x line*=bottom
      	  ]
                \addplot[fill=blue!60] coordinates {
                  (1,10000) % q-A1-untuned.sql
                  (2,10000) % q-A4-untuned.sql
                  (3,10000) % q-A1-untuned.sql
                  (4,10000) % q-A4-untuned.sql
                };
      	  %\label{untuned}
      	  \addplot[draw=black, pattern color = black, pattern = horizontal lines] coordinates {
                  (1,10000) % q-A1-tuned-selfJoin.sql
                  (2,10000) % q-A4-tuned-selfJoin.sql
                  (3,10000) % q-A1-untuned.sql
                  (4,10000) % q-A4-untuned.sql
      	  };
                %\label{tuned-self}
                \addplot[draw=red, pattern color = red, pattern = north west lines] coordinates {
                  (1,10000) % q-A1-tuned-full.sql
                  (2,10000) % q-A4-tuned-full.sql
                  (3,10000) % q-A1-untuned.sql
                  (4,10000) % q-A4-untuned.sql
                };
          
              \end{axis}        
      	\begin{axis}[
                  at=(bottom axis.north),
                  anchor=south, yshift=\pgfkeysvalueof{/tikz/axis break gap},
      	    ybar=0pt,
                  bar width=0.1cm,
                  %title=\textsc{Wisconsin 100M},
      	    height=3.5cm,
      	    width=4cm,
            	    xtick={1,2},
            	    xticklabels={$q_{A1}^p$,$q_{A1}^d$,$q_{A4}^p$,$q_{A4}^d$},
      	    ytick={10000,100000,1000000},
                  yticklabels={10s, 100s, 20m},
      	    grid=major,
      	    legend columns=-1,
                  ymin=10000, 
      	    ymax=1200000,
                  ymode=log,
                  xticklabel=\empty,
                  axis x line*=top, %% remove the top line
                  after end axis/.code={
                    \draw (rel axis cs:0,0) +(-1mm,-1mm) -- +(1mm,1mm)
                    ++(0pt,-\pgfkeysvalueof{/tikz/axis break gap})
                    +(-1mm,-1mm) -- +(1mm,1mm)
                    (rel axis cs:1,0) +(-1mm,-1mm) -- +(1mm,1mm)
                    ++(0pt,-\pgfkeysvalueof{/tikz/axis break gap})
                    +(-1mm,-1mm) -- +(1mm,1mm);
                  }
      	  ]
	  
      	  \addplot[fill=blue!60] coordinates {
                  (1,610813) % q-A1^p-untuned.sql
                  (2,431548) % q-A1^d-untuned.sql
            
                  (3,1200000) % q-A4^p-untuned.sql
                  (4,1200000) % q-A4^d-untuned.sql (69 minutes)
      	  };
      	  \label{wis-cte-untuned}
      	  \addplot[draw=black, pattern color = black, pattern = horizontal lines] coordinates {
                  (1,45977)  % q-A1^p-tuned-selfjoin.sql
                  (2,159930) % q-A1^d-tuned-selfjoin.sql
            
                  (3,45552) % q-A4^p-tuned-selfJoin.sql
                  (4,82091) % q-A4^d-tuned-selfJoin.sql
      	  };
                \label{wis-cte-tuned-self}
                \addplot[draw=red, pattern color = red, pattern = north west lines] coordinates {
                  (1,46003) % q-A1^p-tuned-full.sql
                  (2,80703) % q-Aq^d-tuned-full.sql
            
            
                  (3,45469) % q-A4-tuned-full.sql
                  (4,84526) % q-A4^d-tuned-full.sql
            
      	  };
                \label{wis-cte-tuned-full}
      	\end{axis}
            \end{tikzpicture}
          \end{minipage}
          %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        &
    %\centering
    \hspace{-7ex}
    \begin{minipage}{.14\textwidth}
     % \hspace{-4ex}
      \begin{tikzpicture}
	\pgfplotsset{every axis/.append style={
	    font=\scriptsize,
	    semithick,
	    tick style={thick}}}
	% FishMark - Results
        \begin{axis}[
            name=bottom axis,
	    ybar=0pt,
            bar width=0.1cm,
	    height=2cm,
	    width=5cm,
      	    xtick={1,2,3,4,5,6},
      	    xticklabels={$q_{6}^p$,$q_{6}^{d}$,$q_{11}^p$,$q_{11}^{d}$,$q_{12}^p$,$q_{12}^{d}$},
	    ytick=\empty,
            yticklabels=\empty,
	    grid=major,
	    legend columns=-1,
            ymin=0, 
	    ymax=10000,
            %ymode=log,
            axis x line*=bottom
	  ]

          \addplot[fill=blue!60] coordinates {
            (1,10000) % q-06-untuned.sql
            (3,10000) % q-11-untuned.sql
            (5,10000) % q-12-untuned.sql

            (2,10000) % q-06-untuned db2
            (4,10000) % q-11-untuned db2
            (6,10000) % q-12-untuned db2
	  };
	  %\label{untuned}
	  \addplot[draw=black, pattern color = black, pattern = horizontal lines] coordinates {
            (1,10000) % q-06-tuned-selfJoin.sql
            (3,10000) % q-11-tuned-selfJoin.sql
            (5,10000) % q-12-tuned-selfJoin.sql

            (2,10000) % q-06-tuned-selfjoin.sql db2
            (4,10000) % q-11-tuned-self db2
            (6,10000) % q-12-tuned-self db2
	  };
          %\label{tuned-self}
          \addplot[draw=red, pattern color = red, pattern = north west lines] coordinates {
            (1,10000) % q-06-tuned-full.sql
            (3,10000) % q-11-tuned-full.sql
            (5,10000) % q-12-tuned-full.sql

            (2,10000) % q-06-tuned-full.sql db2
            (4,10000) % q-11-tuned-full db2
            (6,10000) % q-12-tuned-full db2
            
	  };
          
        \end{axis}
	\begin{axis}[
            at=(bottom axis.north),
            anchor=south, yshift=\pgfkeysvalueof{/tikz/axis break gap},
	    ybar=0pt,
            bar width=0.1cm,
            %ylabel={\scriptsize Query exec. time (ms.)},
	    height=3.5cm,
	    width=5cm,
      	    xtick={1,2,3,4,5,6},
      	    %xticklabels={$q_{6}^p$,$q_{6}^{d}$,$q_{11}^p$,$q_{11}^{d}$,$q_{12}^p$,$q_{12}^{d}$},
	    %ytick={10000,100000,1000000},
	    grid=major,
            %title=\textsc{NPD\_10},
            legend columns=-1,
            ymin=10000, 
	    ymax=1200000,
            yticklabels={10s, 100s, 20m},
            ymode=log,
            xticklabel=\empty,
            axis x line*=top, %% remove the top line
            after end axis/.code={
              \draw (rel axis cs:0,0) +(-1mm,-1mm) -- +(1mm,1mm)
              ++(0pt,-\pgfkeysvalueof{/tikz/axis break gap})
              +(-1mm,-1mm) -- +(1mm,1mm)
              (rel axis cs:1,0) +(-1mm,-1mm) -- +(1mm,1mm)
              ++(0pt,-\pgfkeysvalueof{/tikz/axis break gap})
              +(-1mm,-1mm) -- +(1mm,1mm);
            }
	  ]
	  
	  \addplot[fill=blue!60] coordinates {
            (1,32867) % q-06-untuned.sql
            (3,126346) % q-11-untuned.sql
            (5,525873) % q-12-untuned.sql

            (2,19788) % q-06-untuned db2
            (4,107433) % q-11-untuned db2
            (6,100370) % q-12-untuned db2
	  };
	  \label{npd-untuned}
	  \addplot[draw=black, pattern color = black, pattern = horizontal lines] coordinates {
            (1,31236) % q-06-tuned-selfJoin.sql
            (3,1200000) % q-11-tuned-selfJoin.sql
            (5,1200000) % q-12-tuned-selfJoin.sql

            (2,20060) % q-06-tuned-selfjoin.sql db2
            (4,107245) % q-11-tuned-self db2
            (6,102182) % q-12-tuned-self db2
	  };
          \label{npd-tuned-self}
          \addplot[draw=red, pattern color = red, pattern = north west lines] coordinates {
            (1,15920) % q-06-tuned-full.sql
            (3,113192) % q-11-tuned-full.sql
            (5,95301) % q-12-tuned-full.sql

            (2,12867) % q-06-tuned-full.sql db2
            (4,54369) % q-11-tuned-full db2
            (6,52148) % q-12-tuned-full db2
            
	  };
          \label{npd-tuned-full}
          
	\end{axis}
      \end{tikzpicture}
    \end{minipage}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
  \begin{minipage}{.5\textwidth}
    \centering
    %\hspace{.20\textwidth}
    \scriptsize{
      \ref{npd-untuned} No CTE~~~ 
      \ref{npd-tuned-self} CTE~~~
      \ref{npd-tuned-full} CTE-\vfd~~~
    }
\end{minipage}
  %&  
  %\begin{minipage}{.2\textwidth}
    %\centering
  %  \hspace{.12\textwidth}
  %  \footnotesize{
  %    \ref{untuned} None~~~ 
  %    \ref{tuned-self} CTE-Self~~~
  %    \ref{tuned-full} CTE-Full~~~
  %  }
  %\end{minipage}
%\end{tabular}





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../../main"
%%% End:


==> graphs/cte/wisconsin/wisc-cte-graph.tex <==
\begin{center}
  \begin{figure}
  \begin{tabular}{c}
    \begin{tabular}{c}
      \begin{minipage}{.5\textwidth}
        %\centering
        \hspace{.13\textwidth}
	\begin{tikzpicture}
	  \pgfplotsset{every axis/.append style={
	      font=\footnotesize,
	      semithick,
	      tick style={thick}}}
	  % FishMark - Results
	  \begin{axis}[
	      ybar=0pt,
              bar width=0.1cm,
              title=\textsc{Wisconsin 100M},
	      height=5cm,
	      %width=4cm,
      	      xtick={1,2},
      	      xticklabels={$q_{A1}$,$q_{A4}$},
	      ytick={10,1000,10000,100000,1000000},
	      grid=major,
	      legend columns=-1,
              %ymin=1, 
	      %ymax=1000000,
              ymode=log
	    ]
	    
	    \addplot[fill=blue!60] coordinates {
              (1,610813) % q-A1-untuned.sql
              (2,4046402) % q-A4-untuned.sql
	    };
	    \label{untuned}
	    \addplot[draw=black, pattern color = black, pattern = horizontal lines] coordinates {
              (1,45977)  % q-A1-tuned-selfjoin.sql
              (2,45552) % q-A4-tuned-selfJoin.sql
	    };
            \label{tuned-self}
            \addplot[draw=red, pattern color = red, pattern = north west lines] coordinates {
              (1,46003) % q-A1-tuned-full.sql
              (2,45469) % q-A4-tuned-full.sql
	    };
            \label{tuned-full}
	  \end{axis}
	\end{tikzpicture}
      \end{minipage}
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \end{tabular}
    \\	
    \begin{minipage}{.5\textwidth}
      %\centering
      \hspace{.15\textwidth}
      \footnotesize{
	\ref{untuned} UNF~~~ 
	\ref{tuned-self} CTE-Self~~~
        \ref{tuned-full} CTE-Full~~~
      }
    \end{minipage}
  \end{tabular}
  
  \caption{CTE Tuning on Wisconsin100M}
  \label{fig:ontopVsStardog}	
\end{figure}
\end{center}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> graphs/old/graph-mysql-int.tex <==
	\begin{tabular}{c}
	
	\begin{tabular}{cc}
		\begin{minipage}{.30\textwidth}
		\begin{tikzpicture}
		\pgfplotsset{every axis/.append style={
			font=\footnotesize,
			semithick,
			tick style={thick}}}
			% FishMark - Results
		    \begin{axis}[
				title= MySQL,
	    			height=7cm,
				width=14cm,
				xtick={0,1,2,3,4,5,6,7,8,9,10,11,12},
				xticklabels={0,1,2,3,4,5,6,7,8,9,10,11,12},
		        	grid=major,
				ymode=log,
				% legend to name=benchmarkset,
				legend columns=-1
		    ]
%%%%%%%%%%%%%%%%%%%%%%%    
   	     %JOINS !!
%%%%%%%%%%%%%%%%%%%%%%%
\addplot[black,mark=square, mark options={solid}] coordinates { (1,128)(2,7)(3,6)(4,10)(5,9)(6,18)(7,24)(8,7)(9,15)(10,8)(11,8)(12,6) };
\addplot[black,mark=triangle, mark options={solid}] coordinates { (1,20)(2,13)(3,8)(4,20)(5,9)(6,20)(7,19)(8,9)(9,22)(10,8)(11,11)(12,9) };
\addplot[black,mark=o, mark options={solid}] coordinates { (1,22)(2,10)(3,14)(4,20)(5,7)(6,17)(7,20)(8,7)(9,21)(10,7)(11,11)(12,13) };
\addplot[black,mark=ball, mark options={solid}] coordinates { (1,22)(2,8)(3,13)(4,23)(5,8)(6,15)(7,9)(8,14)(9,27)(10,9)(11,10)(12,12) };
\addplot[black,mark=diamond, mark options={solid}] coordinates { (1,32)(2,8)(3,16)(4,18)(5,10)(6,7)(7,13)(8,8)(9,22)(10,7)(11,13)(12,7) };
\addplot[black,mark=otimes, mark options={solid}] coordinates { (1,138)(2,12)(3,24)(4,110)(5,18)(6,25)(7,34)(8,13)(9,28)(10,15)(11,12)(12,15) };
%%%%%%%%%%%%%%%%%%%%%%%
    %View no keys!!!
%%%%%%%%%%%%%%%%%%%%%%%
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=square, mark options={solid}] coordinates { (1,314)(2,211)(3,224)(4,207)(5,249)(6,270)(7,268)(8,292)(9,318)(10,275)(11,297)(12,331) };
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=triangle, mark options={solid}] coordinates { (1,157)(2,186)(3,237)(4,179)(5,204)(6,263)(7,185)(8,224)(9,283)(10,189)(11,232)(12,289) };
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=o, mark options={solid}] coordinates { (1,172)(2,209)(3,277)(4,178)(5,227)(6,306)(7,194)(8,249)(9,326)(10,198)(11,249)(12,330) };
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=ball, mark options={solid}] coordinates { (1,249)(2,390)(3,630)(4,260)(5,406)(6,681)(7,272)(8,420)(9,669)(10,274)(11,430)(12,672) };
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=diamond, mark options={solid}] coordinates { (1,363)(2,608)(3,1053)(4,363)(5,634)(6,1152)(7,373)(8,648)(9,1088)(10,377)(11,647)(12,1100) };
\addplot[black,dash pattern=on 3pt off 6pt on 6pt off 6pt,mark=otimes, mark options={solid}] coordinates { (1,2257)(2,4610)(3,8862)(4,2165)(5,4617)(6,9702)(7,2177)(8,4633)(9,8784)(10,2159)(11,4647)(12,8878) };
%%%%%%%%%%%%%%%%%%%%%%%
    %View Tuned keys!!!
%%%%%%%%%%%%%%%%%%%%%%%
\addplot[black,densely dotted,mark=square, mark options={solid}] coordinates { (1,425)(2,359)(3,103)(4,385)(5,390)(6,173)(7,492)(8,156)(9,149)(10,626)(11,164)(12,174) };
\addplot[black,densely dotted,mark=triangle, mark options={solid}] coordinates { (1,48)(2,46)(3,44)(4,45)(5,50)(6,48)(7,57)(8,65)(9,52)(10,47)(11,51)(12,69) };
\addplot[black,densely dotted,mark=o, mark options={solid}] coordinates { (1,61)(2,45)(3,45)(4,138)(5,46)(6,49)(7,43)(8,47)(9,51)(10,53)(11,57)(12,58) };
\addplot[black,densely dotted,mark=ball, mark options={solid}] coordinates { (1,54)(2,51)(3,87)(4,59)(5,49)(6,57)(7,51)(8,55)(9,56)(10,48)(11,56)(12,56) };
\addplot[black,densely dotted,mark=diamond, mark options={solid}] coordinates { (1,58)(2,41)(3,67)(4,78)(5,46)(6,52)(7,59)(8,51)(9,60)(10,56)(11,53)(12,63) };
\addplot[black,densely dotted,mark=otimes, mark options={solid}] coordinates { (1,223)(2,45)(3,71)(4,86)(5,55)(6,63)(7,57)(8,55)(9,62)(10,60)(11,66)(12,60) };
\end{axis}
\end{tikzpicture}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& 

	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
\\	
\begin{minipage}{.90\textwidth}
	\centering
		\footnotesize{
			\ref{mil} $\sigma_{1.000}$~~~ 
			\ref{diez} $\sigma_{10.000}$ ~~~
			\ref{veinte} $\sigma_{20.000}$~~~
			\ref{cincuenta} $\sigma_{50.000}$~~~
			\ref{cien} $\sigma_{100.000}$ ~~~
			\ref{quinientos} $\sigma_{500.000}$ ~~~
			}
\end{minipage}
\end{tabular}


==> img/macros-tikz.tex <==
\colorlet{rolecolor}{black}
\colorlet{indcolor}{black}
\colorlet{homcolor}{gray}

\colorlet{tboxcolor}{blue}
\colorlet{aboxcolor}{yellow}

\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}


\pgfmathparse{atan2(0,1)}
\ifdim\pgfmathresult pt=0pt % atan2(y, x)
  \tikzset{declare function={atanXY(\x,\y)=atan2(\y,\x);atanYX(\y,\x)=atan2(\y,\x);}}
\else                       % atan2(x, y)
  \tikzset{declare function={atanXY(\x,\y)=atan2(\x,\y);atanYX(\y,\x)=atan2(\x,\y);}}
\fi


\tikzset{ %
  %%% node styles
  %
  abox/.style={cylinder, shape border rotate=90, aspect=0.2, outer sep=0.05cm,
    draw, fill=aboxcolor},%
  aboxl/.style={abox, draw=aboxcolor!60, fill=aboxcolor!20},%
  aboxr/.style={abox},%
  %
  abox3d/.style={abox, drop shadow, draw=aboxcolor!90!black, %
    left color=aboxcolor!70, right color=aboxcolor!80, middle color=white,%
    append after command={ let%
      \p{cyl@center} = ($(\tikzlastnode.before top)!0.5!(\tikzlastnode.after top)$), %
      \p{cyl@x} = ($(\tikzlastnode.before top)-(\p{cyl@center})$), %
      \p{cyl@y} = ($(\tikzlastnode.top) -(\p{cyl@center})$) in %
      (\p{cyl@center}) edge[draw=none, fill=aboxcolor!50, to path={ ellipse%
        [x radius=veclen(\p{cyl@x})-1\pgflinewidth-0.05cm, %
        y radius=veclen(\p{cyl@y})-1\pgflinewidth-0.05cm, rotate=atanXY(\p{cyl@x})]}]
      () }%
  },%
  %   abox3dl/.style={aboxl, outer sep=-0.5\pgflinewidth, %
  %   left color=aboxcolor!30, right color=aboxcolor!40, middle color=white,%
  %   postaction={decorate, decoration={markings, mark=at position 0 with%
  %   {\fill[fill=aboxcolor!40] let \p1=($(cyl.before top)!0.5!(cyl.after
  %   top)$), \p2=(cyl.top), \p3=(cyl.before top), %
  %   \n1={veclen(\x3-\x1,\y3-\y1)}, \n2={veclen(\x2-\x1,\y2-\y1)} in %
  %   (\p1) ellipse (\n2 and \n1); }%
  % }}%
  % },%
  %   abox3dr/.style={abox3d}, %
  %
  tbox/.style={thick, outer sep=0.05cm, inner sep=0.2cm, draw, fill=tboxcolor!50},%
  tboxl/.style={tbox, draw=tboxlcolor, fill=tboxlcolor!40}, %
  tboxr/.style={tbox, draw=tboxrcolor, fill=tboxrcolor!40}, %
  %
  tbox3d/.style={tbox, drop shadow={opacity=0.35},
    %draw=tboxcolor!80, inner color=tboxcolor!50, outer  color=tboxcolor!80
    thin, draw=tboxcolor!50, top color=tboxcolor!20, bottom color=tboxcolor!50
  },%
  tbox3dl/.style={tbox, draw=tboxlcolor!60, inner color=tboxrcolor!20, outer
    color=tboxrcolor!40},%
  tbox3dr/.style={tbox, draw=tboxrcolor!85, inner color=tboxrcolor!45, outer
    color=tboxrcolor!65},%
  %
  kbbox/.style={draw, thick, outer sep=0cm, inner sep=0.2cm},%
  kbbox3d/.style={kbbox, outer sep=0.05cm, rounded corners},%
  %
  entity/.style={draw, fill=white, thick, inner xsep=0.2cm, outer sep=0.02cm},%
  relation/.style={draw, diamond, aspect=3, fill=white, thick, inner
    ysep=0.02cm, drop shadow},%
  attribute/.style={draw, circle, fill=white, thick, inner sep=0.07cm},%
  %
  umlclass/.style={rectangle split, rectangle split parts=3, rectangle split
    part align={center, left, left}, draw, thick, drop shadow={opacity=0.3},
    inner ysep=0.05cm, %
    rectangle split empty part height=0.2cm, fill=gray!50},%
  umlclassabstract/.style={rectangle split, rectangle split parts=3, rectangle
    split part align={center, left, left}, draw, thick, drop shadow={opacity=0.3},
    inner ysep=0.05cm, %
    rectangle split empty part height=0.0cm, fill=gray!50},%
  %
  %% canonical model
  individual/.style={draw, circle, outer sep=0.05cm, inner sep=0.08cm, thick,
    color=indcolor, text=indcolor}, %
  constant/.style={fill}, %
  %
  region/.style={rounded corners, color=mygray, fill=mygray!30, text=black}, %
  %
  %%% arrow styles
  %
  isa/.style={-open triangle 60, thick},%
  erisa/.style={decoration={markings,mark=at position 1 with {\arrow[line
        width=0.1cm]{stealth}}}, postaction={decorate}},%
  assoc/.style={thick},%
  %
  role/.style={-stealth', thick, color=rolecolor},%
  disj/.style={triangle 60-triangle 60, fill=white, ultra thin, postaction={decorate,
    decoration={markings, mark=at position 0.45 with {\draw[-,solid]
        (-2pt,-2pt) -- (2pt, 2pt); } }}},%
  %
  trans/.style={-stealth', semithick},%
  homomor/.style={-stealth, dashed, thick, color=homcolor},%
  %
  soledge/.style={dashed,-latex},%
  path/.style={decorate, decoration={zigzag, segment length=20pt,
      amplitude=2pt},->, ultra thin},%
  mapping/.style={decorate, decoration={coil, aspect=0, segment length=20pt,
      amplitude=1pt},-latex, ultra thin, mydarkgray},%
  disjmap/.style={decorate, decoration={coil, aspect=0, segment length=20pt,
      amplitude=1pt},-latex, ultra thin, mydarkgray, postaction={decorate,
    decoration={markings, mark=at position 0.55 with {\draw[-,solid]
        (-2pt,-2pt) -- (2pt, 2pt); } }}},%
  crossout/.style={decorate, decoration={markings, mark=at position 0.55 with
      {\draw[-,solid,thick,myred] (-2pt,-2pt) -- (2pt, 2pt); %
        \draw[-,solid,thick,myred] (-2pt,2pt) -- (2pt, -2pt);} }},%
  %
  isometricYXZ/.style={x={(1cm,0cm)}, y={(-1.299cm,-0.75cm)}, z={(0cm,1cm)}},%
}



\def \tikzdots[#1]{
  \begin{scope}[shift={#1}, text=black, inner sep=0.05cm]
    \node at (0,0.15) {\per}; \node {\per}; \node at (0,-0.15) {\per};
  \end{scope}
}





%% decoration for shifted path
\def\pgfdecoratedcontourdistance{0pt}

\pgfkeys{/pgf/decoration/contour distance/.code={%
    \pgfmathparse{#1}%
    \let\pgfdecoratedcontourdistance=\pgfmathresult}%
}

\pgfdeclaredecoration{contour lineto}{start}
{
    \state{start}[next state=draw, width=0pt]{
        \pgfpathmoveto{\pgfpoint{0pt}{\pgfdecoratedcontourdistance}}%
    }
    \state{draw}[next state=draw, width=\pgfdecoratedinputsegmentlength]{
        \pgfmathparse{-\pgfdecoratedcontourdistance*cot(-\pgfdecoratedangletonextinputsegment/2+90)}%
        \let\shorten=\pgfmathresult%
        \pgfpathlineto{\pgfpoint{\pgfdecoratedinputsegmentlength+\shorten}{\pgfdecoratedcontourdistance}}%
    }
    \state{final}{
        \pgfpathlineto{\pgfpoint{\pgfdecoratedinputsegmentlength}{\pgfdecoratedcontourdistance}}%
    }
}


% #1 number of teeths
% #2 radius intern
% #3 radius extern
% #4 angle from start to end of the first arc
% #5 angle to decale the second arc from the first
% #6 inner radius to cut off
\newcommand{\gear}[6]{%
  (0:#2)
  \foreach \i [evaluate=\i as \n using {\i-1)*360/#1}] in {1,...,#1}{%
    arc (\n:\n+#4:#2) {[rounded corners=1.5pt] -- (\n+#4+#5:#3)
    arc (\n+#4+#5:\n+360/#1-#5:#3)} --  (\n+360/#1:#2)
  }%
  (0,0) circle[radius=#6]
}




%-----ABoxes
%-----#1 height, #2 width, #3 aspect, #4 name of the node, #5
%-----coordinate, #6 label

\def\aboxl[#1,#2,#3,#4,#5]#6{%
  \node[draw, cylinder, alias=cyl, shape border rotate=90, aspect=#3, %
  minimum height=#1, minimum width=#2, outer sep=-0.5\pgflinewidth, %
  color=aboxcolor!60, left color=aboxcolor!30, right color=aboxcolor!40, middle
  color=white] (#4) at #5 {};%
  %
  \node at #5 {#6};%
  %
  \fill [left color=aboxcolor!20, right color=aboxcolor!20] let \p1 =
  ($(cyl.before top)!0.5!(cyl.after top)$), \p2 = (cyl.top), \p3 = (cyl.before
  top), \n1={veclen(\x3-\x1,\y3-\y1)}, \n2={veclen(\x2-\x1,\y2-\y1)} in (\p1)
  ellipse (\n1 and \n2); }



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main-slides"
%%% TeX-PDF-mode: t
%%% save-place: t
%%% End:

==> img/obda.tex <==
%\begin{center}

%\end{center}

%\begin{center}
  \begin{tikzpicture}[mycloud/.style={draw, shape=cloud, outer sep=0.05cm}]

    %% conceptual layer
    \begin{scope}[shift={(0,5)}]
      \foreach \al/\x/\y in {%
        C1/-0.5/0.75,%
        C2/-1/0,%
        C3/0/0,%
        C4/0.5/0.75,%
        C5/1/0%
      }{ \node[entity, circle, inner sep=0.05cm] (\al) at (\x,\y) {}; }

      \foreach \from/\to in {%
        C1/C2, C2/C3, C3/C1, C1/C4, C4/C5%
      }{ \draw[thick] (\from) -- (\to); }

      \begin{pgfonlayer}{background}
        \node[mycloud, cloud puffs=17, aspect=2, gray, fill=gray!20, dashed,
        inner sep=1.1cm, %
        label={[shift={(1.6cm,-0.75cm)}, gray!50!black]above left:{\small
            Inferred triples}}] (inferred) at (0,0.45) {};%

        \node[mycloud, cloud puffs=13, aspect=2, fill=white, fit=(C1)(C2)(C5),
        yshift=-0.3cm, inner xsep=0.3cm, %
        label={[yshift=0.8cm]below:{\small virtual RDF graph}}] (rdfgraph) {};%

        \node[draw, rounded corners, fit=(inferred)(inferred.puff 9), inner
        xsep=0.8cm, inner ysep=0.3cm, yshift=0.1cm] (conceptlayer) {};

        \node[anchor=north east] at (conceptlayer.north east) {\bf Conceptual Layer};
      \end{pgfonlayer}

      \draw[latex-, thick] (conceptlayer.100) -- node[left] {$\mathbf{q}$} +(0,1);
      \draw[-latex, thick] (conceptlayer.80) -- node[right] {result} +(0,1);
    \end{scope}


    %% mapping
    \begin{scope}[shift={(0,2.1)}]
      \node[draw=gray, fill=gray!50, thick, outer sep=0.05cm, inner ysep=0.5cm,
      inner xsep=1.5cm] (map) at (0,0) {\bf Mapping};
    \end{scope}


    %% resources
    \begin{scope}
      \foreach \al/\x/\y/\lab in {%
        r1/-2/0/{1},%
        r2/-0.5/0/{2},%
        r3/2/0/{n}%
      }{ \node[abox, fill=white] (\al) at (\x,\y) {\begin{minipage}{1.1cm}
            \centering \footnotesize Resource \lab\end{minipage}}; %
        \draw[latex-latex, thick] (\al) -- (map); } \node at (0.75,0) {\dots};
    
      \node[draw, rounded corners, fit=(r1)(r2)(r3), inner xsep=1.38cm, inner
      ysep=0.4cm, yshift=-0.15cm] (datalayer) {};

      \node[anchor=south east] at (datalayer.south east) {\bf Datasources};
    \end{scope}


    %%arrows
    \foreach \from/\to in {%
      r1/map, r2/map, r3/map,%
      rdfgraph.puff 7/map.north-|rdfgraph.puff 7, %
      rdfgraph.puff 8/map.north-|rdfgraph.puff 8%
    }{ \draw[latex-latex, thick] (\from) -- (\to); }

    \draw[-stealth, very thick, dashed, gray, text=black]%
    (conceptlayer.320) -- node[right] {%
      \begin{minipage}{1.2cm}\it query \\translation\end{minipage}
    } (datalayer.north-|conceptlayer.320);

  \end{tikzpicture}
%\end{center}


==> img/obdaWorkflow.tex <==
\noindent\centerline{\begin{tikzpicture}[>=latex]
\node[text width=7em] (q) at (0,1) {\footnotesize SPARQL
query\\[-2pt]\hspace*{1em}{\scriptsize\&} ontology};
\node (qp) at (3,1) {\footnotesize SPARQL query};
\node (ref) at (3,0) {\footnotesize virtual RDF graph};
\draw[->,out=-90,in=180] (q) to node[midway, left, text width=4em]
{\scriptsize entailment\\[-5pt]regime} (ref);
\draw[->,dashed] (qp) to node[midway, right, text width=4em]
{\scriptsize simple\\[-5pt]entailment} (ref);
%
\node (s) at (6,1) {\footnotesize SQL query};
\node (tr) at (6,0) {\footnotesize triple-database};
\draw[->,dashed] (s) to node[midway, right, text width=4em]
{\scriptsize evaluation} (tr);
%
\node (sql) at (9,1) {\footnotesize SQL query};
\node (db) at (9,0) {\footnotesize database};
\draw[->] (sql) to node[midway, right, text width=4em] {\scriptsize
evaluation} (db);
%
\draw[->] (q) to node[above, midway] {\footnotesize $\dagger$} (qp);
\draw[->] (qp) to node[above, midway] {\footnotesize $\boldsymbol{\tau}$} (s);
\draw[->] (s) to node[above, midway] {\scriptsize unfolding} (sql);
%
\draw[->] (db) to node[below, midway] {\scriptsize mapping} (tr);
\draw[->] (tr) to node[below, midway] {\footnotesize $\approx$} (ref);
\end{tikzpicture}}


==> queries/wisconsinDb2.tex <==
\begin{verbatim}
The input SPARQL query:
=======================
PREFIX :	<http://www.example.org/> SELECT ?x ?y  WHERE {?x a  :1Tab1 . ?x :Tab2unique2Tab2 ?y . Filter( ?y < 100 )}

The output SQL query:
=====================
SELECT 
   1 AS "xQuestType", NULL AS "xLang", ('http://www.example.org/' || REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(REPLACE
   (REPLACE(REPLACE(REPLACE(CAST(QVIEW1."unique2Tab1" AS VARCHAR(500)),' ', '%20'),'!', '%21'),'@', '%40'),'#', '%23'),'$', '%24'),'&', '%26'),'*', '%42'), '(', '%28'), ')', '%29'), 
    '[', '%5B'), ']', '%5D'), ',', '%2C'), ';', '%3B'), ':', '%3A'), '?', '%3F'), '=', '%3D'), '+', '%2B'), '''', '%22'), '/', '%2F')) AS "x", 
   4 AS "yQuestType", NULL AS "yLang", CAST(QVIEW2."unique1Tab2" AS VARCHAR(500)) AS "y"
 FROM 
"Tab1" QVIEW1,
"Tab2" QVIEW2
WHERE 
(QVIEW1."unique2Tab1" = QVIEW2."unique2Tab2") AND
QVIEW1."unique2Tab1" IS NOT NULL AND
QVIEW2."unique1Tab2" IS NOT NULL AND
(QVIEW2."unique1Tab2" < 100)

The input SPARQL query:
=======================
PREFIX :	<http://www.example.org/> SELECT ?x ?y  WHERE {?x a  :2Tab1 . ?x :Tab3unique2Tab3 ?y . Filter( ?y < 100 )}

The output SQL query:
=====================
SELECT 
   1 AS "xQuestType", NULL AS "xLang", ('http://www.example.org/' || REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(REPLACE
   (REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(REPLACE(CAST(QVIEW1."unique2Tab1" AS VARCHAR(500)),' ', '%20'),'!', '%21'),'@', '%40'),'#', '%23'),'$', '%24'),'&', '%26'),
   '*', '%42'), '(', '%28'), ')', '%29'), '[', '%5B'), ']', '%5D'), ',', '%2C'), ';', '%3B'), ':', '%3A'), '?', '%3F'), '=', '%3D'), '+', '%2B'), '''', '%22'), '/', '%2F')) AS "x", 
   4 AS "yQuestType", NULL AS "yLang", CAST(QVIEW3."unique1Tab3" AS VARCHAR(500)) AS "y"
 FROM 
"Tab1" QVIEW1,
"Tab2" QVIEW2,
"Tab3" QVIEW3
WHERE 
(QVIEW1."unique2Tab1" = QVIEW2."unique2Tab2") AND
(QVIEW1."unique2Tab1" = QVIEW3."unique2Tab3") AND
QVIEW1."unique2Tab1" IS NOT NULL AND
QVIEW3."unique1Tab3" IS NOT NULL AND
(QVIEW3."unique1Tab3" < 100)
\end{verbatim}


==> tables/intTableDb2100M.tex <==
\begin{tabular}{l \tableColSpace l \tableColSpace l \tableColSpace l \tableColBigSpace l \tableColSpace l \tableColSpace l \tableColBigSpace l \tableColSpace l \tableColSpace l \tableColSpace l}
\toprule
& \multicolumn{3}{l}{Int Joins} & \multicolumn{3}{l}{Int Views No MK} & \multicolumn{3}{l}{Int Views MK} \tableRowBreak
\textit{Queries} & 1 SJ & 2 SJ & 3 SJ & 1 SJ & 2 SJ & 3 SJ & 1 SJ & 2 SJ & 3 SJ & \textit{\# Results}\tableRowBreak
\midrule
\textit{1 SQL Join} \tableRowBreak
$q_{1}$ & 29678 & 29450 & 29493 & 106775 & 196704 & 194935 & 48780 & 48381 & 48126 & 100 \tableRowBreak
$q_{2}$ & 32377 & 32513 & 31859 & 98352 & 213303 & 199867 & 48501 & 48535 & 48234 & 10000 \tableRowBreak
$q_{3}$ & 34134 & 34114 & 34223 & 119687 & 152899 & 227250 & 48860 & 48693 & 48805 & 100000 \tableRowBreak
\textit{2 SQL Joins} \tableRowBreak
$q_{4}$ & 29410 & 29677 & 29581 & 146419 & 202864 & 279444 & 66210 & 66120 & 66352 & 100 \tableRowBreak
$q_{5}$ & 36907 & 36487 & 36872 & 143021 & 206174 & 285294 & 66275 & 65904 & 67038 & 10000 \tableRowBreak
$q_{6}$ & 46690 & 47271 & 47828 & 141722 & 207384 & 290380 & 67263 & 67490 & 67654 & 100000 \tableRowBreak
\textit{3 SQL Joins} \tableRowBreak
$q_{7}$ & 25814 & 25609 & 25538 & 201748 & 291407 & 412515 & 97885 & 97693 & 97702 & 100 \tableRowBreak
$q_{8}$ & 44051 & 40489 & 40623 & 202336 & 292299 & 409188 & 97646 & 97376 & 97671 & 10000 \tableRowBreak
$q_{9}$ & 46789 & 47196 & 46188 & 203960 & 296149 & 410302 & 97755 & 97762 & 97777 & 100000 \tableRowBreak
\textit{4 SQL Joins} \tableRowBreak
$q_{10}$ & 27865 & 27899 & 27586 & 246728 & 349365 & 480299 & 118702 & 118514 & 118835 & 100 \tableRowBreak
$q_{11}$ & 53110 & 54210 & 54155 & 247468 & 349854 & 466107 & 118192 & 119107 & 118175 & 10000 \tableRowBreak
$q_{12}$ & 47570 & 47823 & 49529 & 254598 & 357175 & 473966 & 118323 & 118619 & 118474 & 100000 \tableRowBreak
\bottomrule
\end{tabular}



==> tables/intTableMysql.tex <==
\begin{tabular}{l \tableColSpace l \tableColSpace l \tableColSpace l \tableColBigSpace l \tableColSpace l \tableColSpace l \tableColBigSpace l \tableColSpace l \tableColSpace l \tableColSpace l}
\toprule
& \multicolumn{3}{l}{Int Joins} & \multicolumn{3}{l}{Int Views No MK} & \multicolumn{3}{l}{Int Views MK} \tableRowBreak
\textit{Queries} & 1 SJ & 2 SJ & 3 SJ & 1 SJ & 2 SJ & 3 SJ & 1 SJ & 2 SJ & 3 SJ & \textit{\# Results}\tableRowBreak
\midrule
\textit{1 SQL Join} \tableRowBreak
$q_{1}$ & 10 & 6 & 4 & 314 & 211 & 224 & 425 & 359 & 103 & 1 \tableRowBreak
%$q_{2}$ & 19 & 6 & 4 & 157 & 186 & 237 & 48 & 46 & 44 & 5 \tableRowBreak
%$q_{3}$ & 7 & 6 & 4 & 172 & 209 & 277 & 61 & 45 & 45 & 10 \tableRowBreak
%$q_{4}$ & 14 & 4 & 11 & 249 & 390 & 630 & 54 & 51 & 87 & 50 \tableRowBreak
$q_{2}$ & 19 & 4 & 15 & 363 & 608 & 1053 & 58 & 41 & 67 & 100 \tableRowBreak
$q_{3}$ & 25 & 12 & 25 & 2257 & 4610 & 8862 & 223 & 45 & 71 & 1000 \tableRowBreak
\textit{2 SQL Joins} \tableRowBreak
$q_{4}$ & 3 & 7 & 15 & 207 & 249 & 270 & 385 & 390 & 173 & 1 \tableRowBreak
%$q_{8}$ & 4 & 6 & 13 & 179 & 204 & 263 & 45 & 50 & 48 & 5 \tableRowBreak
%$q_{9}$ & 3 & 4 & 4 & 178 & 227 & 306 & 138 & 46 & 49 & 10 \tableRowBreak
%$q_{10}$ & 11 & 4 & 3 & 260 & 406 & 681 & 59 & 49 & 57 & 50 \tableRowBreak
$q_{5}$ & 6 & 4 & 7 & 363 & 634 & 1152 & 78 & 46 & 52 & 100 \tableRowBreak
$q_{6}$ & 11 & 11 & 20 & 2165 & 4617 & 9702 & 86 & 55 & 63 & 1000 \tableRowBreak
\textit{3 SQL Joins} \tableRowBreak
$q_{7}$ & 4 & 4 & 3 & 268 & 292 & 318 & 492 & 156 & 149 & 1 \tableRowBreak
%$q_{14}$ & 8 & 4 & 5 & 185 & 224 & 283 & 57 & 65 & 52 & 5 \tableRowBreak
%$q_{15}$ & 4 & 4 & 5 & 194 & 249 & 326 & 43 & 47 & 51 & 10 \tableRowBreak
%$q_{16}$ & 5 & 5 & 4 & 272 & 420 & 669 & 51 & 55 & 56 & 50 \tableRowBreak
$q_{8}$ & 5 & 6 & 5 & 373 & 648 & 1088 & 59 & 51 & 60 & 100 \tableRowBreak
$q_{9}$ & 10 & 9 & 10 & 2177 & 4633 & 8784 & 57 & 55 & 62 & 1000 \tableRowBreak
\textit{4 SQL Joins} \tableRowBreak
$q_{10}$ & 5 & 7 & 5 & 275 & 297 & 331 & 626 & 164 & 174 & 1 \tableRowBreak
%$q_{20}$ & 4 & 5 & 3 & 189 & 232 & 289 & 47 & 51 & 69 & 5 \tableRowBreak
%$q_{21}$ & 4 & 5 & 3 & 198 & 249 & 330 & 53 & 57 & 58 & 10 \tableRowBreak
%$q_{22}$ & 6 & 4 & 4 & 274 & 430 & 672 & 48 & 56 & 56 & 50 \tableRowBreak
$q_{11}$ & 4 & 5 & 4 & 377 & 647 & 1100 & 56 & 53 & 63 & 100 \tableRowBreak
$q_{12}$ & 10 & 9 & 9 & 2159 & 4647 & 8878 & 60 & 66 & 60 & 1000 \tableRowBreak
\bottomrule
\end{tabular}



==> tables/intTablePostgres.tex <==
\begin{tabular}{l \tableColSpace l \tableColSpace l \tableColSpace l \tableColBigSpace l \tableColSpace l \tableColSpace l \tableColBigSpace l \tableColSpace l \tableColSpace l \tableColSpace l}
\toprule
& \multicolumn{3}{l}{Int Joins} & \multicolumn{3}{l}{Int Views No MK} & \multicolumn{3}{l}{Int Views MK} \tableRowBreak
\textit{Queries} & 1 SJ & 2 SJ & 3 SJ & 1 SJ & 2 SJ & 3 SJ & 1 SJ & 2 SJ & 3 SJ & \textit{\# Results}\tableRowBreak
\midrule
\textit{1 SQL Join} \tableRowBreak
$q_{1}$ & 47 & 58 & 58 & 136 & 202 & 247 & 84 & 80 & 79 & 1 \tableRowBreak
%$q_{2}$ & 43 & 54 & 58 & 136 & 198 & 242 & 78 & 77 & 81 & 5 \tableRowBreak
%$q_{3}$ & 43 & 52 & 69 & 141 & 200 & 240 & 83 & 79 & 83 & 10 \tableRowBreak
%$q_{4}$ & 49 & 54 & 66 & 141 & 201 & 258 & 85 & 78 & 86 & 50 \tableRowBreak
$q_{2}$ & 50 & 56 & 65 & 145 & 199 & 232 & 83 & 78 & 86 & 100 \tableRowBreak
$q_{3}$ & 155 & 110 & 124 & 203 & 234 & 250 & 139 & 95 & 93 & 1000 \tableRowBreak
\textit{2 SQL Joins} \tableRowBreak
$q_{4}$ & 42 & 54 & 63 & 189 & 269 & 320 & 115 & 113 & 114 & 1 \tableRowBreak
%$q_{8}$ & 42 & 54 & 60 & 189 & 279 & 314 & 116 & 111 & 114 & 5 \tableRowBreak
%$q_{9}$ & 43 & 55 & 60 & 194 & 273 & 303 & 119 & 114 & 114 & 10 \tableRowBreak
%$q_{10}$ & 44 & 56 & 65 & 190 & 259 & 298 & 114 & 124 & 114 & 50 \tableRowBreak
$q_{5}$ & 56 & 59 & 63 & 196 & 335 & 298 & 120 & 117 & 116 & 100 \tableRowBreak
$q_{6}$ & 123 & 199 & 128 & 223 & 283 & 324 & 136 & 127 & 126 & 1000 \tableRowBreak
\textit{3 SQL Joins} \tableRowBreak
$q_{7}$ & 44 & 53 & 59 & 271 & 331 & 428 & 161 & 158 & 153 & 1 \tableRowBreak
%$q_{14}$ & 46 & 53 & 60 & 240 & 319 & 416 & 159 & 161 & 154 & 5 \tableRowBreak
%$q_{15}$ & 41 & 54 & 61 & 242 & 315 & 413 & 149 & 154 & 154 & 10 \tableRowBreak
%$q_{16}$ & 46 & 55 & 62 & 239 & 317 & 413 & 148 & 150 & 153 & 50 \tableRowBreak
$q_{8}$ & 53 & 58 & 64 & 253 & 314 & 411 & 150 & 165 & 153 & 100 \tableRowBreak
$q_{9}$ & 78 & 85 & 91 & 268 & 346 & 442 & 239 & 169 & 165 & 1000 \tableRowBreak
\textit{4 SQL Joins} \tableRowBreak
$q_{10}$ & 43 & 57 & 63 & 308 & 400 & 558 & 192 & 193 & 195 & 1 \tableRowBreak
%$q_{20}$ & 43 & 61 & 63 & 297 & 395 & 563 & 194 & 194 & 194 & 5 \tableRowBreak
%$q_{21}$ & 45 & 56 & 63 & 291 & 393 & 570 & 190 & 195 & 202 & 10 \tableRowBreak
%$q_{22}$ & 45 & 58 & 68 & 308 & 392 & 549 & 187 & 197 & 196 & 50 \tableRowBreak
$q_{11}$ & 47 & 61 & 68 & 294 & 395 & 541 & 189 & 210 & 197 & 100 \tableRowBreak
$q_{12}$ & 121 & 134 & 142 & 331 & 430 & 576 & 207 & 207 & 211 & 1000 \tableRowBreak
\bottomrule
\end{tabular}



==> tables/intTablePostgres100M.tex <==
\begin{tabular}{l \tableColSpace l \tableColSpace l \tableColSpace l \tableColBigSpace l \tableColSpace l \tableColSpace l \tableColBigSpace l \tableColSpace l \tableColSpace l \tableColSpace l}
\toprule
& \multicolumn{3}{l}{Int Joins} & \multicolumn{3}{l}{Int Views No MK} & \multicolumn{3}{l}{Int Views MK} \tableRowBreak
\textit{Queries} & 1 SJ & 2 SJ & 3 SJ & 1 SJ & 2 SJ & 3 SJ & 1 SJ & 2 SJ & 3 SJ & \textit{\# Results}\tableRowBreak
\midrule
\textit{1 SQL Join} \tableRowBreak
$q_{1}$ & 33092 & 34598 & 38261 & 155329 & 233036 & 306822 & 89907 & 80465 & 90164 & 100 \tableRowBreak
$q_{2}$ & 27678 & 34484 & 40699 & 163427 & 247375 & 336214 & 69937 & 55742 & 60105 & 10000 \tableRowBreak
$q_{3}$ & 30642 & 24127 & 27409 & 182725 & 292524 & 402491 & 56241 & 56329 & 59581 & 100000 \tableRowBreak
\textit{2 SQL Joins} \tableRowBreak
$q_{4}$ & 35061 & 40628 & 44010 & 237939 & 357133 & 470173 & 127478 & 123473 & 126394 & 100 \tableRowBreak
$q_{5}$ & 24739 & 31019 & 40902 & 244957 & 374701 & 492976 & 127168 & 124025 & 125039 & 10000 \tableRowBreak
$q_{6}$ & 26378 & 23936 & 28180 & 264017 & 407329 & 549186 & 127661 & 125387 & 129507 & 100000 \tableRowBreak
\textit{3 SQL Joins} \tableRowBreak
$q_{7}$ & 31183 & 36326 & 39715 & 301614 & 450355 & 596186 & 160994 & 158965 & 166706 & 100 \tableRowBreak
$q_{8}$ & 33443 & 38412 & 46703 & 313454 & 467451 & 621753 & 162318 & 161768 & 166713 & 10000 \tableRowBreak
$q_{9}$ & 26845 & 25084 & 30571 & 330196 & 498662 & 671774 & 160228 & 164210 & 163476 & 100000 \tableRowBreak
\textit{4 SQL Joins} \tableRowBreak
$q_{10}$ & 39456 & 42505 & 43226 & 484799 & 710921 & 944842 & 258756 & 256198 & 262414 & 100 \tableRowBreak
$q_{11}$ & 58470 & 55836 & 64043 & 497433 & 737316 & 984687 & 258567 & 258160 & 260859 & 10000 \tableRowBreak
$q_{12}$ & 54460 & 37987 & 61322 & 514041 & 778225 & 1037260 & 262777 & 263927 & 261882 & 100000 \tableRowBreak
\bottomrule
\end{tabular}



==> tables/strTableMysql.tex <==
\begin{tabular}{l \tableColSpace l \tableColSpace l \tableColSpace l \tableColBigSpace l \tableColSpace l \tableColSpace l \tableColBigSpace l \tableColSpace l \tableColSpace l \tableColSpace l}
\toprule
& \multicolumn{3}{l}{Int Joins} & \multicolumn{3}{l}{Int Views No MK} & \multicolumn{3}{l}{Int Views MK} \tableRowBreak
\textit{Queries} & 1 SJ & 2 SJ & 3 SJ & 1 SJ & 2 SJ & 3 SJ & 1 SJ & 2 SJ & 3 SJ & \textit{\# Results}\tableRowBreak
\midrule
\textit{1 SQL Join} \tableRowBreak
$q_{1}$ & 8 & 10 & 5 & 680 & 370 & 391 & 457 & 223 & 98 & 1 \tableRowBreak
$q_{2}$ & 6 & 11 & 4 & 309 & 376 & 466 & 47 & 44 & 46 & 5 \tableRowBreak
$q_{3}$ & 6 & 4 & 15 & 343 & 453 & 596 & 53 & 44 & 49 & 10 \tableRowBreak
$q_{4}$ & 14 & 6 & 9 & 545 & 971 & 1640 & 65 & 42 & 86 & 50 \tableRowBreak
$q_{5}$ & 15 & 4 & 6 & 802 & 1667 & 2917 & 59 & 44 & 77 & 100 \tableRowBreak
$q_{6}$ & 17 & 8 & 10 & 5400 & 13749 & 26046 & 194 & 51 & 66 & 1000 \tableRowBreak
\textit{2 SQL Joins} \tableRowBreak
$q_{7}$ & 9 & 5 & 4 & 513 & 395 & 463 & 394 & 142 & 185 & 1 \tableRowBreak
$q_{8}$ & 7 & 4 & 4 & 353 & 406 & 469 & 75 & 46 & 52 & 5 \tableRowBreak
$q_{9}$ & 5 & 10 & 5 & 369 & 459 & 570 & 46 & 48 & 58 & 10 \tableRowBreak
$q_{10}$ & 6 & 5 & 5 & 572 & 885 & 1291 & 61 & 49 & 63 & 50 \tableRowBreak
$q_{11}$ & 5 & 6 & 5 & 823 & 1402 & 2233 & 89 & 50 & 51 & 100 \tableRowBreak
$q_{12}$ & 11 & 10 & 9 & 5295 & 11006 & 18824 & 85 & 56 & 62 & 1000 \tableRowBreak
\textit{3 SQL Joins} \tableRowBreak
$q_{13}$ & 4 & 3 & 5 & 610 & 446 & 523 & 515 & 159 & 144 & 1 \tableRowBreak
$q_{14}$ & 7 & 3 & 3 & 410 & 433 & 513 & 154 & 56 & 54 & 5 \tableRowBreak
$q_{15}$ & 5 & 4 & 4 & 425 & 489 & 596 & 50 & 59 & 54 & 10 \tableRowBreak
$q_{16}$ & 6 & 5 & 4 & 601 & 879 & 1306 & 59 & 59 & 61 & 50 \tableRowBreak
$q_{17}$ & 4 & 5 & 3 & 813 & 1385 & 2203 & 63 & 60 & 60 & 100 \tableRowBreak
$q_{18}$ & 9 & 8 & 10 & 4699 & 10407 & 18265 & 70 & 68 & 64 & 1000 \tableRowBreak
\textit{4 SQL Joins} \tableRowBreak
$q_{19}$ & 5 & 4 & 4 & 495 & 523 & 582 & 618 & 140 & 152 & 1 \tableRowBreak
$q_{20}$ & 8 & 4 & 3 & 407 & 471 & 549 & 48 & 55 & 56 & 5 \tableRowBreak
$q_{21}$ & 4 & 3 & 2 & 430 & 521 & 634 & 52 & 62 & 57 & 10 \tableRowBreak
$q_{22}$ & 5 & 5 & 5 & 598 & 914 & 1343 & 51 & 57 & 59 & 50 \tableRowBreak
$q_{23}$ & 4 & 5 & 6 & 815 & 1423 & 2237 & 50 & 56 & 63 & 100 \tableRowBreak
$q_{24}$ & 9 & 9 & 10 & 4681 & 10482 & 18387 & 55 & 66 & 69 & 1000 \tableRowBreak
\bottomrule
\end{tabular}



==> tables/strTablePostgres.tex <==
\begin{tabular}{l \tableColSpace l \tableColSpace l \tableColSpace l \tableColBigSpace l \tableColSpace l \tableColSpace l \tableColBigSpace l \tableColSpace l \tableColSpace l \tableColSpace l}
\toprule
& \multicolumn{3}{l}{Int Joins} & \multicolumn{3}{l}{Int Views No MK} & \multicolumn{3}{l}{Int Views MK} \tableRowBreak
\textit{Queries} & 1 SJ & 2 SJ & 3 SJ & 1 SJ & 2 SJ & 3 SJ & 1 SJ & 2 SJ & 3 SJ & \textit{\# Results}\tableRowBreak
\midrule
\textit{1 SQL Join} \tableRowBreak
$q_{1}$ & 42 & 43 & 52 & 173 & 256 & 321 & 88 & 93 & 87 & 1 \tableRowBreak
$q_{2}$ & 41 & 41 & 53 & 177 & 254 & 316 & 87 & 92 & 88 & 5 \tableRowBreak
$q_{3}$ & 43 & 39 & 61 & 181 & 253 & 308 & 90 & 91 & 90 & 10 \tableRowBreak
$q_{4}$ & 45 & 42 & 57 & 176 & 252 & 324 & 94 & 91 & 99 & 50 \tableRowBreak
$q_{5}$ & 51 & 43 & 59 & 181 & 252 & 310 & 96 & 95 & 96 & 100 \tableRowBreak
$q_{6}$ & 167 & 116 & 148 & 244 & 275 & 344 & 150 & 108 & 122 & 1000 \tableRowBreak
\textit{2 SQL Joins} \tableRowBreak
$q_{7}$ & 43 & 38 & 53 & 224 & 316 & 420 & 109 & 108 & 111 & 1 \tableRowBreak
$q_{8}$ & 41 & 39 & 54 & 228 & 315 & 413 & 119 & 188 & 111 & 5 \tableRowBreak
$q_{9}$ & 43 & 39 & 54 & 222 & 309 & 403 & 116 & 116 & 109 & 10 \tableRowBreak
$q_{10}$ & 48 & 42 & 58 & 234 & 314 & 392 & 117 & 113 & 115 & 50 \tableRowBreak
$q_{11}$ & 50 & 46 & 60 & 233 & 314 & 388 & 132 & 119 & 114 & 100 \tableRowBreak
$q_{12}$ & 160 & 147 & 158 & 260 & 347 & 431 & 143 & 137 & 127 & 1000 \tableRowBreak
\textit{3 SQL Joins} \tableRowBreak
$q_{13}$ & 42 & 42 & 56 & 287 & 397 & 545 & 153 & 150 & 150 & 1 \tableRowBreak
$q_{14}$ & 43 & 42 & 56 & 275 & 395 & 546 & 143 & 156 & 150 & 5 \tableRowBreak
$q_{15}$ & 43 & 42 & 56 & 294 & 392 & 550 & 143 & 143 & 146 & 10 \tableRowBreak
$q_{16}$ & 54 & 47 & 60 & 286 & 393 & 542 & 146 & 141 & 151 & 50 \tableRowBreak
$q_{17}$ & 59 & 50 & 64 & 287 & 407 & 534 & 152 & 143 & 151 & 100 \tableRowBreak
$q_{18}$ & 164 & 165 & 175 & 315 & 440 & 581 & 160 & 158 & 163 & 1000 \tableRowBreak
\textit{4 SQL Joins} \tableRowBreak
$q_{19}$ & 50 & 44 & 61 & 337 & 476 & 637 & 180 & 180 & 189 & 1 \tableRowBreak
$q_{20}$ & 46 & 50 & 59 & 343 & 486 & 629 & 187 & 179 & 186 & 5 \tableRowBreak
$q_{21}$ & 46 & 47 & 60 & 343 & 492 & 633 & 185 & 182 & 187 & 10 \tableRowBreak
$q_{22}$ & 51 & 50 & 64 & 335 & 492 & 629 & 182 & 179 & 196 & 50 \tableRowBreak
$q_{23}$ & 56 & 55 & 69 & 335 & 489 & 627 & 191 & 182 & 193 & 100 \tableRowBreak
$q_{24}$ & 190 & 188 & 204 & 376 & 514 & 682 & 205 & 196 & 213 & 1000 \tableRowBreak
\bottomrule
\end{tabular}



==> tables/strTablePostgres100M.tex <==
\begin{tabular}{l \tableColSpace l \tableColSpace l \tableColSpace l \tableColBigSpace l \tableColSpace l \tableColSpace l \tableColBigSpace l \tableColSpace l \tableColSpace l \tableColSpace l}
\toprule
& \multicolumn{3}{l}{Int Joins} & \multicolumn{3}{l}{Int Views No MK} & \multicolumn{3}{l}{Int Views MK} \tableRowBreak
\textit{Queries} & 1 SJ & 2 SJ & 3 SJ & 1 SJ & 2 SJ & 3 SJ & 1 SJ & 2 SJ & 3 SJ & \textit{\# Results}\tableRowBreak
\midrule
\textit{1 SQL Join} \tableRowBreak
$q_{1}$ & 100 \tableRowBreak
$q_{2}$ & 10000 \tableRowBreak
$q_{3}$ & 100000 \tableRowBreak
$q_{4}$ \tableRowBreak
$q_{5}$ \tableRowBreak
$q_{6}$ \tableRowBreak
\textit{2 SQL Joins} \tableRowBreak
$q_{7}$ & 100 \tableRowBreak
$q_{8}$ & 10000 \tableRowBreak
$q_{9}$ & 100000 \tableRowBreak
$q_{10}$ \tableRowBreak
$q_{11}$ \tableRowBreak
$q_{12}$ \tableRowBreak
\textit{3 SQL Joins} \tableRowBreak
$q_{13}$ & 100 \tableRowBreak
$q_{14}$ & 10000 \tableRowBreak
$q_{15}$ & 100000 \tableRowBreak
$q_{16}$ \tableRowBreak
$q_{17}$ \tableRowBreak
$q_{18}$ \tableRowBreak
\textit{4 SQL Joins} \tableRowBreak
$q_{19}$ & 100 \tableRowBreak
$q_{20}$ & 10000 \tableRowBreak
$q_{21}$ & 100000 \tableRowBreak
$q_{22}$ \tableRowBreak
$q_{23}$ \tableRowBreak
$q_{24}$ \tableRowBreak
\bottomrule
\end{tabular}



==> tables/table-db2-em.tex <==
\begin{tabular}{c c c c c c c c c c c c c c c c c c c c}
  \toprule
  \multicolumn{5}{c}{Group 1} & \multicolumn{5}{c}{Group 2} & \multicolumn{5}{c}{Group3} & \multicolumn{5}{c}{Group 4} \tableRowBreak
  \#C & id & depth & idF & time & \#C & id & depth & idF & time & \#C & id & depth & idF & time & \#C & id & depth & idF & time \tableRowBreak
  \midrule
0 & 0 & 0 & 0 & 33527 &0 & 0 & 0 & 0 & 27807 &0 & 0 & 0 & 0 & 28217 &0 & 0 & 0 & 0 & 27550 \tableRowBreak
0 & 1 & 0 & 1 & 86311 &0 & 1 & 0 & 1 & 69854 &0 & 1 & 0 & 1 & 69756 &0 & 1 & 0 & 1 & 69824 \tableRowBreak 
0 & 2 & 0 & 2 & 123655 &0 & 2 & 0 & 2 & 97094 &0 & 2 & 0 & 2 & 97074 &0 & 2 & 0 & 2 & 97694 \tableRowBreak
0 & 3 & 1 & 0 & 128841 &0 & 3 & 1 & 0 & 27893 &0 & 3 & 1 & 0 & 27616 &0 & 3 & 1 & 0 & 28474 \tableRowBreak
0 & 4 & 1 & 1 & 171165 &0 & 4 & 1 & 1 & 70646 &0 & 4 & 1 & 1 & 69985 &0 & 4 & 1 & 1 & 69997 \tableRowBreak
0 & 5 & 1 & 2 & 229689 &0 & 5 & 1 & 2 & 100276 &0 & 5 & 1 & 2 & 100835 &0 & 5 & 1 & 2 & 100430 \tableRowBreak
0 & 6 & 2 & 0 & 83420 &0 & 6 & 2 & 0 & 55988 &0 & 6 & 2 & 0 & 28011 &0 & 6 & 2 & 0 & 28701 \tableRowBreak
0 & 7 & 2 & 1 & 208022 &0 & 7 & 2 & 1 & 139946 &0 & 7 & 2 & 1 & 71035 &0 & 7 & 2 & 1 & 70378 \tableRowBreak
0 & 8 & 2 & 2 & 298449 &0 & 8 & 2 & 2 & 198467 &0 & 8 & 2 & 2 & 101596 &0 & 8 & 2 & 2 & 102338 \tableRowBreak
0 & 9 & 3 & 0 & 111242 &0 & 9 & 3 & 0 & 83343 &0 & 9 & 3 & 0 & 55023 &0 & 9 & 3 & 0 & 29618 \tableRowBreak
0 & 10 & 3 & 1 & 278382 &0 & 10 & 3 & 1 & 207156 &0 & 10 & 3 & 1 & 138744 &0 & 10 & 3 & 1 & 66956 \tableRowBreak
0 & 11 & 3 & 2 & 392677 &0 & 11 & 3 & 2 & 295666 &0 & 11 & 3 & 2 & 191658 &0 & 11 & 3 & 2 & 93988 \tableRowBreak
1 & 0 & 0 & 0 & 109606 &1 & 0 & 0 & 0 & 55704 &1 & 0 & 0 & 0 & 56375 &1 & 0 & 0 & 0 & 55591 \tableRowBreak
1 & 1 & 0 & 1 & 307928 &1 & 1 & 0 & 1 & 194367 &1 & 1 & 0 & 1 & 190950 &1 & 1 & 0 & 1 & 194331 \tableRowBreak
1 & 2 & 0 & 2 & 364945 &1 & 2 & 0 & 2 & 183478 &1 & 2 & 0 & 2 & 184580 &1 & 2 & 0 & 2 & 185598 \tableRowBreak
1 & 3 & 1 & 0 & 322876 &1 & 3 & 1 & 0 & 108963 &1 & 3 & 1 & 0 & 58139 &1 & 3 & 1 & 0 & 54821 \tableRowBreak
1 & 4 & 1 & 1 & 948546 &1 & 4 & 1 & 1 & 316375 &1 & 4 & 1 & 1 & 202291 &1 & 4 & 1 & 1 & 201219 \tableRowBreak
1 & 5 & 1 & 2 & 1137312 &1 & 5 & 1 & 2 & 386069 &1 & 5 & 1 & 2 & 199153 &1 & 5 & 1 & 2 & 198475 \tableRowBreak
1 & 6 & 2 & 0 & 632877 &1 & 6 & 2 & 0 & 322994 &1 & 6 & 2 & 0 & 112162 &1 & 6 & 2 & 0 & 55992 \tableRowBreak
1 & 7 & 2 & 1 & 1200043 &1 & 7 & 2 & 1 & 1057514 &1 & 7 & 2 & 1 & 333692 &1 & 7 & 2 & 1 & 218115 \tableRowBreak
1 & 8 & 2 & 2 & 1200029 &1 & 8 & 2 & 2 & 1131471 &1 & 8 & 2 & 2 & 382875 &1 & 8 & 2 & 2 & 200417 \tableRowBreak
1 & 9 & 3 & 0 & 853889 &1 & 9 & 3 & 0 & 473515 &1 & 9 & 3 & 0 & 217776 &1 & 9 & 3 & 0 & 55079 \tableRowBreak
1 & 10 & 3 & 1 & 1200037 &1 & 10 & 3 & 1 & 1200035 &1 & 10 & 3 & 1 & 634747 &1 & 10 & 3 & 1 & 197692 \tableRowBreak
1 & 11 & 3 & 2 & 1200034 &1 & 11 & 3 & 2 & 1200021 &1 & 11 & 3 & 2 & 733774 &1 & 11 & 3 & 2 & 188496 \tableRowBreak
2 & 0 & 0 & 0 & 469340 &2 & 0 & 0 & 0 & 161270 &2 & 0 & 0 & 0 & 80160 &2 & 0 & 0 & 0 & 83832 \tableRowBreak
2 & 1 & 0 & 1 & 1200026 &2 & 1 & 0 & 1 & 404338 &2 & 1 & 0 & 1 & 240834 &2 & 1 & 0 & 1 & 246810 \tableRowBreak
2 & 2 & 0 & 2 & 1200025 &2 & 2 & 0 & 2 & 1004436 &2 & 2 & 0 & 2 & 522491 &2 & 2 & 0 & 2 & 521600 \tableRowBreak
2 & 3 & 1 & 0 & 951332 &2 & 3 & 1 & 0 & 480684 &2 & 3 & 1 & 0 & 160101 &2 & 3 & 1 & 0 & 79732 \tableRowBreak
2 & 4 & 1 & 1 & 1200032 &2 & 4 & 1 & 1 & 1200023 &2 & 4 & 1 & 1 & 405780 &2 & 4 & 1 & 1 & 251729 \tableRowBreak
2 & 5 & 1 & 2 & 1200024 &2 & 5 & 1 & 2 & 1200025 &2 & 5 & 1 & 2 & 1007987 &2 & 5 & 1 & 2 & 535224 \tableRowBreak
2 & 6 & 2 & 0 & 1200042 &2 & 6 & 2 & 0 & 477831 &2 & 6 & 2 & 0 & 166740 &2 & 6 & 2 & 0 & 86264 \tableRowBreak
2 & 7 & 2 & 1 & 1200036 &2 & 7 & 2 & 1 & 1200024 &2 & 7 & 2 & 1 & 466378 &2 & 7 & 2 & 1 & 299764 \tableRowBreak
2 & 8 & 2 & 2 & 1200041 &2 & 8 & 2 & 2 & 1200020 &2 & 8 & 2 & 2 & 807210 &2 & 8 & 2 & 2 & 289181 \tableRowBreak
2 & 9 & 3 & 0 & 1200068 &2 & 9 & 3 & 0 & 1200056 &2 & 9 & 3 & 0 & 654370 &2 & 9 & 3 & 0 & 82542 \tableRowBreak
2 & 10 & 3 & 1 & 1200090 &2 & 10 & 3 & 1 & 1200061 &2 & 10 & 3 & 1 & 1200041 &2 & 10 & 3 & 1 & 321407 \tableRowBreak
2 & 11 & 3 & 2 & 1200062 &2 & 11 & 3 & 2 & 1200053 &2 & 11 & 3 & 2 & 1200020 &2 & 11 & 3 & 2 & 285703 \tableRowBreak
\bottomrule
\end{tabular}


==> tables/table-pgsql-em.tex <==
\begin{tabular}{c c c c c c c c c c c c c c c c c c c c}
  \toprule
  \multicolumn{5}{c}{Group 1} & \multicolumn{5}{c}{Group 2} & \multicolumn{5}{c}{Group3} & \multicolumn{5}{c}{Group 4} \tableRowBreak
  \#C & id & depth & idF & time & \#C & id & depth & idF & time & \#C & id & depth & idF & time & \#C & id & depth & idF & time \tableRowBreak
  \midrule
0 & 0 & 0 & 0 & 14209 &0 & 0 & 0 & 0 & 14414 &0 & 0 & 0 & 0 & 14233 &0 & 0 & 0 & 0 & 14268 \tableRowBreak
0 & 1 & 0 & 1 & 14010 &0 & 1 & 0 & 1 & 14690 &0 & 1 & 0 & 1 & 13957 &0 & 1 & 0 & 1 & 14060 \tableRowBreak
0 & 2 & 0 & 2 & 14339 &0 & 2 & 0 & 2 & 14829 &0 & 2 & 0 & 2 & 14056 &0 & 2 & 0 & 2 & 13972 \tableRowBreak
0 & 3 & 1 & 0 & 29604 &0 & 3 & 1 & 0 & 14802 &0 & 3 & 1 & 0 & 14107 &0 & 3 & 1 & 0 & 14006 \tableRowBreak
0 & 4 & 1 & 1 & 29621 &0 & 4 & 1 & 1 & 14922 &0 & 4 & 1 & 1 & 14150 &0 & 4 & 1 & 1 & 14183 \tableRowBreak
0 & 5 & 1 & 2 & 29642 &0 & 5 & 1 & 2 & 14938 &0 & 5 & 1 & 2 & 14156 &0 & 5 & 1 & 2 & 14138 \tableRowBreak
0 & 6 & 2 & 0 & 44646 &0 & 6 & 2 & 0 & 29241 &0 & 6 & 2 & 0 & 13987 &0 & 6 & 2 & 0 & 13995 \tableRowBreak
0 & 7 & 2 & 1 & 44082 &0 & 7 & 2 & 1 & 28457 &0 & 7 & 2 & 1 & 13972 &0 & 7 & 2 & 1 & 14146 \tableRowBreak
0 & 8 & 2 & 2 & 44225 &0 & 8 & 2 & 2 & 28174 &0 & 8 & 2 & 2 & 13989 &0 & 8 & 2 & 2 & 14098 \tableRowBreak
0 & 9 & 3 & 0 & 62001 &0 & 9 & 3 & 0 & 41608 &0 & 9 & 3 & 0 & 27753 &0 & 9 & 3 & 0 & 14479 \tableRowBreak
0 & 10 & 3 & 1 & 56072 &0 & 10 & 3 & 1 & 41707 &0 & 10 & 3 & 1 & 28018 &0 & 10 & 3 & 1 & 14226 \tableRowBreak
0 & 11 & 3 & 2 & 55897 &0 & 11 & 3 & 2 & 41735 &0 & 11 & 3 & 2 & 28061 &0 & 11 & 3 & 2 & 14132 \tableRowBreak
1 & 0 & 0 & 0 & 59970 &1 & 0 & 0 & 0 & 30151 &1 & 0 & 0 & 0 & 31885 &1 & 0 & 0 & 0 & 30139 \tableRowBreak
1 & 1 & 0 & 1 & 59522 &1 & 1 & 0 & 1 & 30295 &1 & 1 & 0 & 1 & 33197 &1 & 1 & 0 & 1 & 30735 \tableRowBreak
1 & 2 & 0 & 2 & 60684 &1 & 2 & 0 & 2 & 32030 &1 & 2 & 0 & 2 & 33850 &1 & 2 & 0 & 2 & 32263 \tableRowBreak
1 & 3 & 1 & 0 & 191426 &1 & 3 & 1 & 0 & 62311 &1 & 3 & 1 & 0 & 31604 &1 & 3 & 1 & 0 & 31523 \tableRowBreak
1 & 4 & 1 & 1 & 188430 &1 & 4 & 1 & 1 & 62607 &1 & 4 & 1 & 1 & 31583 &1 & 4 & 1 & 1 & 31681 \tableRowBreak
1 & 5 & 1 & 2 & 193121 &1 & 5 & 1 & 2 & 63952 &1 & 5 & 1 & 2 & 32637 &1 & 5 & 1 & 2 & 32608 \tableRowBreak
1 & 6 & 2 & 0 & 383312 &1 & 6 & 2 & 0 & 190215 &1 & 6 & 2 & 0 & 62955 &1 & 6 & 2 & 0 & 31499 \tableRowBreak
1 & 7 & 2 & 1 & 380969 &1 & 7 & 2 & 1 & 197616 &1 & 7 & 2 & 1 & 63097 &1 & 7 & 2 & 1 & 31673 \tableRowBreak
1 & 8 & 2 & 2 & 387541 &1 & 8 & 2 & 2 & 196158 &1 & 8 & 2 & 2 & 65302 &1 & 8 & 2 & 2 & 32918 \tableRowBreak
1 & 9 & 3 & 0 & 480133 &1 & 9 & 3 & 0 & 281685 &1 & 9 & 3 & 0 & 126714 &1 & 9 & 3 & 0 & 31360 \tableRowBreak
1 & 10 & 3 & 1 & 498237 &1 & 10 & 3 & 1 & 294317 &1 & 10 & 3 & 1 & 126621 &1 & 10 & 3 & 1 & 33187 \tableRowBreak
1 & 11 & 3 & 2 & 532850 &1 & 11 & 3 & 2 & 296751 &1 & 11 & 3 & 2 & 129952 &1 & 11 & 3 & 2 & 34425 \tableRowBreak
2 & 0 & 0 & 0 & 32596 &2 & 0 & 0 & 0 & 31513 &2 & 0 & 0 & 0 & 31607 &2 & 0 & 0 & 0 & 33598 \tableRowBreak
2 & 1 & 0 & 1 & 50777 &2 & 1 & 0 & 1 & 48404 &2 & 1 & 0 & 1 & 48335 &2 & 1 & 0 & 1 & 49470 \tableRowBreak
2 & 2 & 0 & 2 & 51275 &2 & 2 & 0 & 2 & 48707 &2 & 2 & 0 & 2 & 48750 &2 & 2 & 0 & 2 & 50819 \tableRowBreak
2 & 3 & 1 & 0 & 31416 &2 & 3 & 1 & 0 & 31655 &2 & 3 & 1 & 0 & 31525 &2 & 3 & 1 & 0 & 32964 \tableRowBreak
2 & 4 & 1 & 1 & 48656 &2 & 4 & 1 & 1 & 46978 &2 & 4 & 1 & 1 & 49066 &2 & 4 & 1 & 1 & 50398 \tableRowBreak
2 & 5 & 1 & 2 & 48912 &2 & 5 & 1 & 2 & 46431 &2 & 5 & 1 & 2 & 50902 &2 & 5 & 1 & 2 & 50693 \tableRowBreak
2 & 6 & 2 & 0 & 297610 &2 & 6 & 2 & 0 & 29844 &2 & 6 & 2 & 0 & 32912 &2 & 6 & 2 & 0 & 32898 \tableRowBreak
2 & 7 & 2 & 1 & 391494 &2 & 7 & 2 & 1 & 45852 &2 & 7 & 2 & 1 & 49235 &2 & 7 & 2 & 1 & 48975 \tableRowBreak
2 & 8 & 2 & 2 & 393685 &2 & 8 & 2 & 2 & 46949 &2 & 8 & 2 & 2 & 49408 &2 & 8 & 2 & 2 & 49308 \tableRowBreak
2 & 9 & 3 & 0 & 1200068 &2 & 9 & 3 & 0 & 1200062 &2 & 9 & 3 & 0 & 351465 &2 & 9 & 3 & 0 & 48219 \tableRowBreak
2 & 10 & 3 & 1 & 1200038 &2 & 10 & 3 & 1 & 1200056 &2 & 10 & 3 & 1 & 391323 &2 & 10 & 3 & 1 & 48605 \tableRowBreak
2 & 11 & 3 & 2 & 1200065 &2 & 11 & 3 & 2 & 1200037 &2 & 11 & 3 & 2 & 399286 &2 & 11 & 3 & 2 & 50076 \tableRowBreak
\bottomrule
\end{tabular}


==> tikz-macros.tex <==
\usepackage{tikz}
\usetikzlibrary{positioning,arrows,fit,snakes}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{calc}
\usetikzlibrary{patterns}
\usetikzlibrary{shapes,shadows}

\tikzset{
  sshadow/.style={opacity=.25, shadow xshift=0.05, shadow yshift=-0.06},
}

%-----#1 size, #2 angle, #3 aspect, #4 label next to the diamond
%-----#5 name of the node, #6 coordinate, #7 label
\def\schemel[#1,#2,#3,#4,#5,#6]#7{ %
  \node[draw, diamond, shape aspect=#3, rotate=#2, minimum size=#1, %
  bottom color=green!55, top color=green!25, color=green!65!black, %
  drop shadow={sshadow,color=green!60!black}, #4] (#5) at #6
  {\textcolor{green!40}{bla}}; %
  \node at #6 {#7};%
}

\def\schemer[#1,#2,#3,#4,#5,#6]#7{ %
  \node[draw, diamond, shape aspect=#3, rotate=#2, minimum size=#1, %
  bottom color=green!65, top color=green!30, color=green!60!black, %
  drop shadow={sshadow,color=green!65!black}, #4] (#5) at #6
  {\textcolor{green!53}{bla}}; %
  \node at #6 {#7}; %
}

%-----TBoxes
%-----#1 height, #2 width, #3 anchor for the label, #4 name of the node, #5
%-----coordinate, #6 label
\def\tboxl[#1,#2,#3,#4,#5]#6{%
  \node[draw, drop shadow={opacity=.35}, minimum height=#1, minimum width=#2, %
  inner color=blue!45, outer color=blue!55, color=blue!40!black] (#4)
at #5 {}; %
  \node[anchor=#3,inner sep=2pt] at (#4.#3) {#6};%
}

\def\tboxr[#1,#2,#3,#4,#5]#6{%
  \node[draw, drop shadow={opacity=.35}, minimum height=#1, minimum width=#2, %
  inner color=blue!35, outer color=blue!45, color=blue!50!black] (#4)
at #5 {}; %
  \node[anchor=#3,inner sep=2pt] at (#4.#3) {#6}; %
}

%-----#1 name of the node, #2 coordinate, #3 label
\def\entity[#1,#2]#3;{
  \node[draw,drop shadow={opacity=.4,shadow xshift=0.04, shadow
    yshift=-0.04},color=blue!30!black,fill=white,rounded corners=3]
(#1) at #2 {#3};
}

%-----#1 from node, #2 to node, #3 specification of a node (label), #4
%-----dashed, or other parameters for draw
\def\isaedge[#1,#2,#3,#4];{
  \draw[-triangle 60,color=black!20!black,#4,fill=white] (#1) -- #3
  (#2);
}

%-----ABoxes
%-----#1 height, #2 width, #3 aspect, #4 name of the node, #5
%-----coordinate, #6 label
\def\aboxl[#1,#2,#3,#4,#5]#6{%
  \node[draw, cylinder, alias=cyl, shape border rotate=90, aspect=#3, %
  minimum height=#1, minimum width=#2, outer sep=-0.5\pgflinewidth, %
  color=orange!40!black, left color=orange!70, right color=orange!80, middle
  color=white] (#4) at #5 {};%
  \node at #5 {#6};%
  \fill [orange!30] let \p1 = ($(cyl.before top)!0.5!(cyl.after top)$), \p2 =
  (cyl.top), \p3 = (cyl.before top), \n1={veclen(\x3-\x1,\y3-\y1)},
  \n2={veclen(\x2-\x1,\y2-\y1)} in (\p1) ellipse (\n1 and \n2); }

\def\aboxr[#1,#2,#3,#4,#5]#6{%
  \node[draw, cylinder, alias=cyl, shape border rotate=90, aspect=#3, %
  minimum height=#1, minimum width=#2, outer sep=-0.5\pgflinewidth, %
  color=black!10!black, left color=black!10, right color=black!10, middle
  color=white] (#4) at #5 {};%
  \node at #5 {#6};%
  \fill [black!20] let \p1 = ($(cyl.before top)!0.5!(cyl.after top)$), \p2 =
  (cyl.top), \p3 = (cyl.before top), \n1={veclen(\x3-\x1,\y3-\y1)},
  \n2={veclen(\x2-\x1,\y2-\y1)} in (\p1) ellipse (\n1 and \n2); }

%-----#1 height, #2 width, #3 name of the node, #4
%-----coordinate, #5 label
\def\kbbox[#1,#2,#3,#4,#5]#6{
        \draw[dashed] node[draw,color=gray!50,minimum
        height=#1,minimum width=#2] (#4) at #5 {};
        \node[anchor=#3,inner sep=2pt] at (#4.#3)  {#6};
}

